Task-Oriented GNNs Training on Large Knowledge Graphs for Accurate and Efficient Modeling

A Knowledge Graph (KG) is a heterogeneous graph encompassing a diverse range of node and edge types. Heterogeneous Graph Neural Networks (HGNNs) are popular for training machine learning tasks like node classification and link prediction on KGs. However, HGNN methods exhibit excessive complexity influenced by the KG's size, density, and the number of node and edge types. AI practitioners handcraft a subgraph of a KG G relevant to a specific task. We refer to this subgraph as a task-oriented subgraph (TOSG), which contains a subset of task-related node and edge types in G. Training the task using TOSG instead of G alleviates the excessive computation required for a large KG. Crafting the TOSG demands a deep understanding of the KG's structure and the task's objectives. Hence, it is challenging and time-consuming. This paper proposes KG-TOSA, an approach to automate the TOSG extraction for task-oriented HGNN training on a large KG. In KG-TOSA, we define a generic graph pattern that captures the KG's local and global structure relevant to a specific task. We explore different techniques to extract subgraphs matching our graph pattern: namely (i) two techniques sampling around targeted nodes using biased random walk or influence scores, and (ii) a SPARQL-based extraction method leveraging RDF engines' built-in indices. Hence, it achieves negligible preprocessing overhead compared to the sampling techniques. We develop a benchmark of real KGs of large sizes and various tasks for node classification and link prediction. Our experiments show that KG-TOSA helps state-of-the-art HGNN methods reduce training time and memory usage by up to 70% while improving the model performance, e.g., accuracy and inference time.

==> Algorithms/GA-FS_Meta_Sampling.tex <==
\begin{algorithm}[t]	\caption{GA-FS Meta-Sampling}
	\label{alg:GA-FS_MS}
	\begin{algorithmic}[1]
	    \Require \textit{Knowledge graph KG; Graph ML task $\mathcal{A}$; Population size n.}
	    \Ensure Knowledge graph \(KG^\prime\).
	    \Function{GA-FS\_MS }{KG,$\mathcal{A}$,n}:
     \State $pop\_var=\infty, Fitness=[]$, $bits =|KG.\mathcal{R}|//2$ 
     \State $population = init\_population(bits,n)$
     
     \While {pop\_var>1}
        \For {i = 1 to n}
            \State $I=getIndividual(i,population)$
            \State $I_{KG}=\textrm{extractSubgraph}(I,KG)$
            \State $Fitness[i]=\textrm{trainGNN}(\mathcal{A},I_{KG})$
        \EndFor          
        \State pop\_var= calcPopVariance(Fitness) 
        \State parents=parentsSelection(population, Fitness)
        \State population = crossoverMutation(population, parents) 
     \EndWhile
     \State $KG'=\textrm{extractSubgraph}(best(population),KG)$
    \EndFunction
\end{algorithmic} 
\end{algorithm} 


==> Algorithms/NR_Meta_Sampling.tex <==
\begin{algorithm}[t]	\caption{VR Meta-Sampling}
	\label{alg:NR_MS}
	\begin{algorithmic}[1]
	    \Require Knowledge graph KG; Graph ML task $\mathcal{A}$; Walk length $h$; batch size $bs$;
     a vertex ranking model $VRM$; a threshold $k$.
	    \Ensure Knowledge graph \(KG^\prime\).
	    \Function{VR-MS }{KG, $\mathcal{A}$, h, bs, $VRM$, $k$}:
	  \State $sg \leftarrow \text{uniformlySampleNodes} (KG,h,bs)$
   \State $\mathcal{V}_l \leftarrow \text{labelTargetNodes }(sg.\mathcal{V}_s,\mathcal{A}.\mathcal{V}_T)$
	            
		\State $\mathcal{V}_{rank} \leftarrow \text{predictVertexRank}(\mathcal{V}_l,VRM)$.
            \State $\mathcal{V}_k \leftarrow \text{getTopVertices }(\mathcal{V}_{rank}, k)$ 
            \State $ KG^\prime \leftarrow  \text{filterOutSubgraph }(\mathcal{V}_k, sg) $
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 


==> Algorithms/Sparql_MS_old.tex <==
\begin{algorithm}[t]	\caption{SPARQL-based Meta-Sampling}
	\label{alg:SPARQL_MS}
	\begin{algorithmic}[1]
	    \Require \textit{Knowledge graph ID $KG_{ID}$; Graph ML task $\mathcal{A}$; Number of Direction $d$ hops $h$; SPARQL Endpoint $SP$.}
	    \Ensure Knowledge graph \(KG'\).
	    \Function{SPARQL\_MS}{$KG_{ID}$, $\mathcal{A}$, $d$, $h$, $SP$}:
      \State$ \mathcal{C}^T_{uri} \leftarrow \textrm{get\_TargetNode\_URIs(}KG_{uri}, RDF_{p}, \mathcal{A}.\mathcal{C}^T).$ 
      \State$ KG^\prime \leftarrow []$
      \For {$c^T_{uri} \in \mathcal{C}^T_{uri}$}
	    \State$ Q_{TCGP} \leftarrow \textrm{write\_TCGP\_Query(}KG_{uri}, c^T_{uri}, h, d).$  
     \State$ v^T_{KG} \leftarrow \textrm{execute\_Query(}RDF_{p}, Q_{TCGP}).$  
     \State $KG^\prime \leftarrow KG^\prime \cup v^T_{KG}$     
     \EndFor
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/CSV_To_GNN.tex <==
\begin{algorithm}[t]
	\caption{CSV To GNN Dataset Transformation}
	\label{alg:CSV_To_GNN}
	\begin{algorithmic}[1]
	    \Require \textit{KG, Target nodes $\mathcal{V}_T$, Target nodes labels $O_T$, User Preferences UPref }
	    \Ensure GNN dataset as a zipped file.
	    \Function{Transform\_KG\_Triples }{KG,$\mathcal{V}_T$,$O_T$,$UPref$}:
	    % \State $dic_{mappings}  \leftarrow \{\} $ \textbf{dictionary of node mappings to ids}.
     %         \State $dic_{AdjMs}  \leftarrow \{\} $ \textbf{dictionary of adjacency matrices}.
     %         \State $dic_{splits}  \leftarrow \{\} $ \textbf{dictionary of dataset splits}.
     \State $dic_{mappings}  \leftarrow \{\} $,
             $dic_{AdjMs}  \leftarrow \{\} $, 
             $dic_{splits}  \leftarrow \{\} $. 
		\For {$c \in \mathcal{C}$}
            \State $dic_{mappings}[c] \leftarrow encode(getV_c(V,c))$
            \EndFor
            \State $dic_{mappings}['label2index'] \leftarrow encode(O_T)$
            \State $dic_{splits} \leftarrow split(encode(V_T),UPref.split)$            
            \For {$r \in R$}             
            \For {$r_{c1},C1,r_{c2} \in getRNodeTypes(KG,r)$}
            \State $dic_{AdjMs}[(r_{c1},r,r_{c2})] \leftarrow AdjM(KG,(r_{c1},r,r_{c2}))$
            \EndFor	
		\EndFor  
            \State write\_csv($dic_{mappings}$,
            $dic_{splits}$,$dic_{AdjMs}$,
            $(V_T,O_T)$)
            \State zipAllDirectories()
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/CSV_To_GNN_old.tex <==
\begin{algorithm}[t]
	\caption{CSV To GNN Dataset Transformation}
	\label{alg:CSV_To_GNN}
	\begin{algorithmic}[1]
	    \Require \textit{KG, Target nodes $\mathcal{V}_T$, Target nodes labels $O_T$ }
	    \Ensure GNN dataset as a zipped file.
	    \Function{Transform\_KG\_Triples }{KG,$\mathcal{V}_T$,$O_T$}:
	    \State $dic_{mappings}  \leftarrow \{\} $ \textbf{dictionary of node mappings to ids}.
             \State $dic_{AdjMs}  \leftarrow \{\} $ \textbf{dictionary of adjacency matrices}.
             \State $dic_{splits}  \leftarrow \{\} $ \textbf{dictionary of dataset splits}.
		\For {$c \in \mathcal{C}$}
            \State $V_c \leftarrow getV_c(V,c)$
            \State $V_c \leftarrow sort(V_c)$
            \State $V_{c-mapping} \leftarrow encode(V_c)$
            \State $dic_{mappings}[c] \leftarrow (V_c,V_{c-mapping})$
            \EndFor
            \State $labels_{Ids} \leftarrow (O_T,encode(sort(O_T))$
            \State $dic_{mappings}['label2index'] \leftarrow (O_T,labels_{Ids})$
            \State $dic_{splits} \leftarrow split(encode(V_T),Random)$
            
            \For {$r \in R$}             
            \State  $C1,C2 \leftarrow getRNodeTypes(KG,r)$
            \For {$r_{c1} \in C1,r_{c2} \in C2$}
		\State  $S,P,O \leftarrow getTriples(KG,(r_{c1},r,r_{c2}))$
            \State  $S_{Ids} \leftarrow getNodeId(S,dic_{mappings})$
            \State  $O_{Ids} \leftarrow getNodeId(O,dic_{mappings})$
            \State  $Adj_c_1rc_2 \leftarrow Build\_AdjM(S_{Ids},O_{Ids})$
            \State $dic_{AdjMs}[(r_{c1},r,r_{c2})] \leftarrow Adj_c_1rc_2$
            \EndFor	
		\EndFor  
            \State $V_{TLabel} \leftarrow (V_T,labels_{Ids})$
            
            \State write($dic_{mappings}$,'mapping')
            \State write($dic_{splits}$,'split/random')
            \State write($dic_{AdjMs}$,'raw/relations')
            \State write($V_{TLabel}$,'raw/node-label')
            \State zipAllDirectories()
		\EndFunction
	\end{algorithmic} 

\end{algorithm} 

==> Algorithms/old_algo/RW.tex <==
\begin{algorithm}[t]
	\caption{Random-walk (RW) sampler \cite{GraphSAINT}}
	\label{alg:RW}
	\begin{algorithmic}[1]
	    \Require \textit{Training graph G (V, E); the number of root nodes r; random walk length h.}
	    \Ensure Sampled graph \( G_s(V_s, E_s)\).
	    \Function{Random\_Walk }{G,r,h}:
	    \State $V_{root}  \leftarrow t$ \textbf{root nodes sampled uniformly at random (with replacement)}.
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
		\State $u \leftarrow v$
		\For {d = 1 to h}
		\State  u ← Node sampled uniformly from u’s neighbor.
		\State  $V_s \leftarrow V_s \cup \{u\}$
		\EndFor
		\EndFor
		\State $G_s \leftarrow $ Node induced sub-graph of $G$ from $V_s$
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/algo_BGP_PQ.tex <==
\begin{algorithm}[t]
	\caption{{\sysName} node classification path-query pattern}
	\label{alg:NC_SQ}
	\begin{algorithmic}[1]
	    \Require \textit{Knoweldge graph KG, Target node type $c_T$.}
	    \Ensure Meta-sampled knoweldge graph \(KG^{\prime} (V^{\prime}, R^\prime)\).
	    \Function{Path\_query\_NC\_Meta-Sampler }{KG,$c_T$}:
	    \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type t from V}.
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
            \State $N_u \leftarrow Out\_Neighbours(v)$
            \State $N_u \leftarrow N_u \cup Out\_Neighbours(N_u)$
            \For {$n \in N_u$}
		\State  $V_s \leftarrow V_s \cup \{n\}$
		\EndFor
		\EndFor            
            \State $ \(KG^\prime \leftarrow Node\) induced sub-graph of G from V_s.$
            \End
		\EndFunction
	\end{algorithmic} 
 %        \begin{algorithmic}[1]
	%     \Function{Bi-directional\_Path\_query\_Sampler}{G,t}:
	%     \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type t from V}.
	%     \State $V_s \leftarrow V_{root}$
	% 	\For {$v \in V_{root}$}
 %            \State $N_{out} \leftarrow Out\_Neighbours(v)$
 %            \State $N_{out} \leftarrow N_{out} \cup Out\_Neighbours(N_{out})$
 %            \State $N_{in} \leftarrow In\_Neighbours(v)$
 %            \State $N_u \leftarrow N_{out} \cup N_{in} \cup In\_Neighbours(N_{in})$
            
 %            \For {$n \in N_u$}
	% 	\State  $V_s \leftarrow V_s \cup \{n\}$
	% 	\EndFor
	% 	\EndFor            
 %            \State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s.$
 %            \End
	% 	\EndFunction
	% \end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/algo_BGP_SQ.tex <==
\begin{algorithm}[t]
	\caption{{\sysName} node classification star-query pattern}
	\label{alg:NC_SQ}
	\begin{algorithmic}[1]
	    \Require \textit{Knoweldge graph KG, Target node type $c_T$.}
	    \Ensure Meta-sampled knoweldge graph \(KG^{\prime} (V^{\prime}, R^\prime)\).
	    \Function{Star\_query\_NC\_Meta-Sampler }{KG,$c_T$}:
	    \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type $c_T$ from V}.
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
            \State $N_u \leftarrow Out\_Neighbours(v)$
            \For {$n \in N_u$}
		\State  $V_s \leftarrow V_s \cup \{n\}$
		\EndFor
		\EndFor            
            \State $ \(KG^\prime \leftarrow Node\) induced sub-graph of G from V_s.$
            \End
		\EndFunction
	\end{algorithmic} 
 %        \begin{algorithmic}[1]
	%     \Function{Bi-directional\_Star\_query\_Sampler }{G,t}:
	%     \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type t from V}.
	%     \State $V_s \leftarrow V_{root}$
	% 	\For {$v \in V_{root}$}
 %            \State $N_u \leftarrow Out\_Neighbours(v)$
 %            \State $N_u \leftarrow N_u \cup In\_Neighbours(v)$
 %            \For {$n \in N_u$}
	% 	\State  $V_s \leftarrow V_s \cup \{n\}$
	% 	\EndFor
	% 	\EndFor            
 %            \State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s.$
 %            \End
	% 	\EndFunction
	% \end{algorithmic} 
 \end{algorithm}
 
%  \begin{algorithm}[t]
% 	\caption{graph patterns selector (1-hop) on knowledge graphs}
% 	\label{alg:P-BP-BGPs}
%         \begin{algorithmic}[1]
%             \Require \textit{Training graph G (V, E); Target node type URI t.}
%             \Ensure Sampled graph \(G_t (V_t, E_t)\).
% 	    \Function{Path\_query\_Sampler}{G,t}:
% 	    \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type t from V}.
% 	    \State $V_s \leftarrow V_{root}$
% 		\For {$v \in V_{root}$}
%             \State $N_u \leftarrow Out\_Neighbours(v)$
%             \State $N_u \leftarrow N_u \cup Out\_Neighbours(N_u)$
%             \For {$n \in N_u$}
% 		\State  $V_s \leftarrow V_s \cup \{n\}$
% 		\EndFor
% 		\EndFor            
%             \State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s.$
%             \End
% 		\EndFunction
% 	\end{algorithmic} 
%         \begin{algorithmic}[1]
% 	    \Function{Bi-directional\_Path\_query\_Sampler}{G,t}:
% 	    \State $V_{root}  \leftarrow r$ \textbf{root nodes are all nodes of type t from V}.
% 	    \State $V_s \leftarrow V_{root}$
% 		\For {$v \in V_{root}$}
%             \State $N_{out} \leftarrow Out\_Neighbours(v)$
%             \State $N_{out} \leftarrow N_{out} \cup Out\_Neighbours(N_{out})$
%             \State $N_{in} \leftarrow In\_Neighbours(v)$
%             \State $N_u \leftarrow N_{out} \cup N_{in} \cup In\_Neighbours(N_{in})$
            
%             \For {$n \in N_u$}
% 		\State  $V_s \leftarrow V_s \cup \{n\}$
% 		\EndFor
% 		\EndFor            
%             \State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s.$
%             \End
% 		\EndFunction
% 	\end{algorithmic} 
% \end{algorithm} 

==> Algorithms/old_algo/algo_biased_sampler.tex <==

\begin{algorithm}[t]
	\caption{Biased random-walk (BRWS) Meta-Sampler}
	\label{alg:BRW}
	\begin{algorithmic}[1]
	    \Require \textit{Training graph G (V, E); target nodes set t; the number of target nodes t; random walk length h.}
	    \Ensure Sampled graph \(G_t (V_t, E_t)\).
	    \Function{Biased\_Random\_Walk }{G,t,h}:
	    \State $V_{root}  \leftarrow t$ \textbf{root nodes sampled uniformly at random (with replacement) from target nodes t}.
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
		\State $u \leftarrow v$
		\For {d = 1 to h}
		\State  u ← Node sampled uniformly from u’s neighbor.
		\State  $V_s \leftarrow V_s \cup \{u\}$
		\EndFor
		\EndFor
		\State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s$
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/algo_weighted_sampler.tex <==

\begin{algorithm}[t]
	\caption{Vertex-Types Ranking Meta-Sampling}
	\label{alg:WRWS}
	\begin{algorithmic}[1]
	    \Require \textit{Training graph G(V, E); W is a population of n weighted node-type items; random walk length h; b batch size.}
	    \Ensure Sampled graph \(G_w (V_w, E_w)\).
	    \Function{Weighted\_Random\_Walk }{G,W,h,b}:
	    % \State $V_{root}  \leftarrow V_s$ \textbf{nodes sampled with respect to nodes-types weights W (with replacement) from all nodes}.
            \State $V_{root} \leftarrow \{\}$
            \For {i=1 to |W|}
            \State $S_i  \leftarrow$ Randomly select an $(W_i.weight*b)$ 
                items from the node type $W_i.type$ 
            \State Insert $S_i$ into $V_{root}$
            \EndFor
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
		\State $u \leftarrow v$
		\For {d = 1 to h}
		\State  u ← Node sampled uniformly from u’s neighbor.
		\State  $V_s \leftarrow V_s \cup \{u\}$
		\EndFor
		\EndFor
		\State $ \(G_s \leftarrow Node\) induced sub-graph of G from V_s$
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 

==> Algorithms/old_algo/learnable-sampler.tex <==
\begin{algorithm}[t]	\caption{Vertex Ranking Meta-Sampling}
	\label{alg:LSRW}
	\begin{algorithmic}[1]
	    \Require \textit{Training graph G (V, E); target nodes set t; number of roots r, the number of target nodes t; random walk length h, ls pre-trained learnable sampler, k top k nodes percentage.}
	    \Ensure Sampled graph \(G_t (V_t, E_t)\).
	    \Function{Learnable-based\_Nodes\_Sampler }{G,r,t,h,ls}:
	    \State $V_{root}  \leftarrow r$ \textbf{root nodes sampled uniformly at random (with replacement) from V}.
	    \State $V_s \leftarrow V_{root}$
		\For {$v \in V_{root}$}
		\State $u \leftarrow v$
		\For {d = 1 to h}
		\State  u ← Node sampled uniformly from u’s neighbor.
		\State  $V_s \leftarrow V_s \cup \{u\}$
		\EndFor
		\EndFor            
		\State $V\_rank \leftarrow prediect\_nodes\_scores(ls,t,V_s)$.
            \State $G_s \leftarrow get\_topk\_nodes(V\_rank,k)\) induced sub-graph.
            % \End
		\EndFunction
	\end{algorithmic} 
\end{algorithm} 


==> sections/KG-TOSA_ha.tex <==
\subsection{A SPARQL-based Extraction Method}
\label{sec:kg-tosa}
\textcolor{blue}{KG data is normally stored into KG engine where triple indexing is performed to allow fast data retrieval. Existing GML frameworks ~\cite{pytorch-geometric, DGCL} extract the whole KG triples and transform it into an adjacency matrix format to perform HGNN training. Our visionary system KGNET in ~\cite{KGNet,SPARQL_ML} bridges this gap by offloading the sampling step into the KG engine. The sampling of subgraphs matching the $KG'$ graph pattern using BRW and IBS is performed through low node selectivity mechanisms that is complex to implement using SPARQL queries and demands higher retrieval complexity. We intended to design carefully a lightweight task oriented sampling method using a high selectivity SPARQL queries that preserve the TOSG characteristics, achieve comparable model performance to BRW and IBS, and avoid costly full data migration outside the KG engine. Thus, we consider BRW and IBS as a baseline to assess the relative performance, efficiency, and effectiveness of our SPAQRL-based method. }

\textcolor{blue}{Our general graph pattern for $KG'$ illustrated in Figure~\ref{fig:node-BGP-samplers} is a basic graph pattern (BGP), which could be performed as a SPARQL query. This pattern preserve: \myNum{i} the local graph structure by considering connected nodes to $\mathcal{V}_T$. \myNum{ii} the global graph structure by interlinking all nodes local structure into a single graph $KG'$. This interlinking allows longer metapaths that is beneficial to meta-path based methods. Furthermore,  the shorter distances between target and non-target nodes allows for constructing multi-layered GCNs with a limited number of hops which save both training time and memory.\shorten
}

Our {\sysName} generates different variations of this query using two main parameters, \myNum{i} predicate direction $d$ and \myNum{ii} the number of hops $h$ to control the node's average distance from target nodes and include various node/edge types. 


In {\sysName}, the BGP query will include by default the outgoing predicates, i.e., $d = 1$, and one hop, $h = 1$ ({\sysName}$_{d1h1}$). Based on the effective mini-batch characteristics in Section~\ref{sec:chars}, TOSG can include three more variations: \myNum{i} ({\sysName}$_{d2h1}$) outgoing and incoming predicates, i.e., $d = 2$, and one hop, $h = 1$,  \myNum{ii} ({\sysName}$_{d1h2}$) outgoing predicates, i.e., $d = 1$, and two hop, $h = 2$, and \myNum{iii} ({\sysName}$_{d2h2}$) outgoing and incoming predicates, i.e., $d = 2$, and two hop, $h = 2$. A SPARQL query ($Q^{d2h1}$) for {\sysName}$_{d2h1}$ could be formulated as:

\begin{figure}[h]
\vspace*{0ex}
  \centering    
  \lstdefinestyle{myStyle}{basicstyle=\small\ttfamily, language=SPARQL }
\begin{lstlisting}    [style=myStyle,captionpos=b,showspaces=false,numbers=left,xleftmargin=0.5cm,morekeywords={v,a,o} ,escapechar=\%,showstringspaces=false,columns=fullflexible]
select ?s ?p ?o {
    select ?v as ?s ?p ?o 
    where { ?v a <Node_Type_URI>.
            ?v ?p ?o.}
    union select ?s ?p ?v as ?o 
    where  {?v a <Node_Type_URI>.
            ?s ?p ?v.} }
\end{lstlisting}
  % \caption{A SPARQL-based query for TCGP with d=2 and h=1.}
  % \label{fig:SPARQL-BGP}
  \vspace*{-2ex}
\end{figure} 


\input{Algorithms/Sparql_MS}

{\sysName} supports all these variations.  
These four variations are used for node classification tasks. 
In the case of a link prediction task targeting vertices of two different types, we add the triple pattern \RDFTYPE{?$v_{Ti}$}{$p_T$}{?$v_{Tj}$} between the two subgraphs extracted for ?$v_{Ti}$ and ?$v_{Tj}$. Algorithm~\ref{alg:SPARQL_MS} is the pseudocode of our SPARQL-based TOSG. It formalizes a BGP for a given task based on a certain $d$ direction and $h$ hops in line 2. However, this query may target a large number of vertices, which can cause issues, e.g., network congestion or low bandwidth. To address this, {\sysName} uses compression and pagination optimization techniques when dealing with query results of a large number of triples. Most RDF engines support compression. Hence, {\sysName} sends an HTTP request to the SPARQL endpoint with a compression flag.

Existing RDF engines support pagination using LIMIT and OFFSET. 
By dividing the results into $k$ mini-batches, most RDF engines will execute the query $k$ times. This is inefficient as our queries are formulated with UNION, such as line 5 in $Q^{d1h1}$. Repeating the UNION query $k$ time is time-consuming due to duplicate elimination. Thus, Algorithm~\ref{alg:SPARQL_MS} paginates each subquery independently. 
Each subquery will benefit from the RDF built-in indices, as the query targets a vertex of a known type.
Existing RDF engines support six indexing schemes for traditional lookup on any subject, predicate or object in a SPARQL query~\cite{Hexastore}.
% ~\cite{Hexastore, TripleBit}
Thus, our SPARQL-based queries are executed efficiently by leveraging the indices existing in RDF engines.\shorten 
%
Algorithm~\ref{alg:SPARQL_MS} collects in $\mathcal{P}$ parallel threads the set of triples in a Pandas DataFrame (DF) and finally uses DF to eliminate duplicates. The algorithm gets as input the batch size per HTTP request. These optimizations are performed in lines 3 to 10.
%
The complexity of {\sysName} is dominated by $\mathcal{QB}$ size in line 7 and the average execution time per query. Also, the drop duplicates step at line 10 is performed in $\mathcal{O}(|KG^{\prime}|)$ which is dominated by the small size of $|KG^{\prime}|$. The $d$ and $h$ parameters contribute to the average query execution time and as well the size of $KG^{\prime}$.

The merging process at line 8 enables {\sysName} to maintain longer metapaths. For example, for the metapath Author-Writes-Paper-Cites-Paper-PublishedIn-Venue in MAG, the subgraphs of common vertices will be interconnected. This process forms a larger sub-graph (TOSG) with longer metapaths while still maintaining a smaller number of hops ($h$) from the target vertices (in this case, vertices of type "Publication"). By using longer metapaths, our method enables HGNNs to achieve better semantic attention. It also allows for constructing multi-layered GCNs with a limited number of hops.
Compared to BRW and IBS, our SPARQL-based method has lower complexity since it does not require sampling on the entire graph and utilizes the RDF engine's built-in indices. This method guarantees to reduce the overall training time and memory usage while improving the model's performance. Hence,  {\sysName} adopts the  SPARQL-based method as the default TOSG extraction method.\shorten





==> sections/ProblemDefination.tex <==
\section{ Problem Definition}
\label{sec:ProblemDefination}

\subsection{The Concept Of Knowledge Graph (KG)}

A knowledge graph refers to a semantic network graph which is consisted of diverse entities, concepts, and relationships in the real world. It is used to formally describe various things and their associations in the real world \cite{Towards_KG,Knowledge_Graphs}. A knowledge graph KG is a tuple (V, E, F, C) where the pairwise disjoint sets V, E, and C correspond to a set of vertices, edges, and classes, respectively.  F represents the fact set, where each fact f is deﬁned as a triple (s,p,o) ${\in}$ F, in which s, p, and o denote the subject entity, the predicate, and the object entity, respectively.

% each statement in KG is modeled as a triple (s,p,o) where s 
% $\in$ V $\cup$ E $\cup$ C, p $\in$ E, and  o $\in$ V $\cup$ E $\cup$ F $\cup$ C.

\subsection{GNN Task on a KG}
\label{bg_ML_Task_Graph}

GNN architectures have been achieving state-of-the-art results in graph machine learning applications,i.e, node classification, graph classification, link prediction, graph clustering, and graph matching \cite{GNN_review_2021}. 
For instance, a node classification problem is commonly applied to graphs to predict an attribute for subset of nodes in a graph, e.g., predict the community or group that a node belongs to in a social network graph \cite{ZhaoYWYD21} or a publishing venue for a paper in a paper citations network KG \cite{OGB}. The inputs for such a task are the graph data, a set of target nodes, and a set of labels (outputs).
Formally, The problem of node classification in KG is to predict statements $(v,e,c)$ that should be in KG, where  $v \in V$ , $e \in E$ denotes the class affiliation relationship, and $c \in C$  is a class. The set of target nodes is denoted by $V^T$ where $V^T \subset V$. 
% $V^T$ can be identified by an RDF \emph{is-a} fact or by a SPARQL query basic graph pattern.

Similarly, the link prediction problem is to predict a missing link or connection between a pair of nodes in a graph, e.g., predict a friendship connection between two users in a social network platform or predict the author of a published paper. The input for this problem is the graph dataset, the set of target node pairs, and the output is the set of true connections. Formally, The problem of link prediction in KG is to predict statements $(v_i,e,v_j)$ that should be in KG, where $v_i \in V^{T}$, $v_j \in V^{T}$ are target nodes, and  $e \in E$  denotes the missing edge(relationship) between the two entities. 
% The target relation r $\in$ R is identified by an RDF URI.
% $V^T$ can be identified by an RDF \emph{is-a} fact or by a SPARQL query basic graph pattern.

\subsection{Meta-Sampling}
Sampling large KGs for GNN training is costly\cite{SamplingSurvey}. The sampling search space is large and the existing task-agnostic (uniform) samplers have a high probability to sample nodes that are not related to the task,i.e, there are nodes/edges that are not good features for the given task to be included during the training, there are isolated nodes that are not connected with any target node so they are useless, there are far away nodes from target nodes or close nodes that are commonly connected with multiple target nodes, these nodes cause over-smoothing\cite{GNN_Over_Smoothing} that drops the training accuracy.
Meta-Sampling is the process of optimizing the uniform sampling process to increase the probability of sampling task-oriented nodes/edges and limit the sampling search space for better scalability.

The Meta-Sampling function takes the knowledge graph KG and the target nodes $V^T$ as input and generates a set of task-oriented sub-graphs as output. We formalized this function in two ways. 

The first formalization is a task-agnostic sampler $S^{TA}$ that uniformly samples a set of sub-graphs $SG=\{sg_1,sg_2,......,sg_n\}$. For each sampled sub-graph $sg_i$ a task-oriented selector fine-tunes the $sg_i$ by dropping out the irrelevant nodes and extracting the $SG^\prime$ subgraph as in (\ref{eq:TB_TA}).
\begin{equation}
\label{eq:TB_TA}
\begin{split}
&SG=S^{TA}(KG),\\
% SG^\prime=S^{TO}(SG,V^T),
&SG^\prime= \{sg^\prime| sg^\prime = S^{TO}(sg,V^T) \text{ where } sg \in SG\}
\\
&GNN\_Train(SG^\prime)
\end{split}
\end{equation}
Where $S^{TO}$ is the task-oriented selector, $S^{TA}$ is the task-agnostic sampler, and $V^T\subset V$ is the set of task target nodes.

The aim is to filter out the less important nodes so the extracted subgraph $SG^\prime \subset SG$ which means a smaller size and hence less training time and memory. The $S^{TO}$ sampler can be replaced with any filtering method such as, ranked node sampler, ranked node-type sampler, and biased node sampler.

The second is a graph task-oriented sampler $S^{TO}$ that extracts a single sub-graph $KG^\prime$ for the given task as a representative of the KG. Then a task-agnostic sampler (uniform sampler) $S^{TA}$ samples the $KG^\prime$ and generates a set of sub-graphs $SG^\prime$ to train the GNN method. Applying the task-oriented sampler once and then applying the uniform sampling as shown in (\ref{eq:TA_TB}), reduces the search space by generating the $KG^\prime \subset KG$.
\begin{equation}
\label{eq:TA_TB}
\begin{split}
&KG^\prime=S^{TO}(KG,V^T),\\
&SG^\prime=S^{TA}(KG^\prime),\\
&GNN\_Train(SG^\prime)
\end{split}
\end{equation}

Where $S^{TO}$ is the task-oriented sampler, $S^{TA}$ is the task-agnostic sampler, and $V^T\subset V$ is the set of target nodes for the given task.
The $S^{TO}$ sampler can be replaced with a feature selector algorithm or a SPARQL query.


% we can define the $S^{TO}$ selector in this case as an edge feature selection optimization problem that selects the best set of nodes/edges that are relevant to the given task.

==> sections/benchmark-oldH.tex <==
\section{Our Open KG Benchmark}
\label{sec:ben}
% To challenge HGNNs on large heterogeneous datasets we introduce a benchmark of various datasets extracted from real KGs. We introduce an overview of our benchmark datasets and discuss the data extraction, the ML tasks and their evaluation metrics and how the train-valid-test splits are created. Then, we present in detail six node classification tasks and two link prediction tasks.

\subsection{An Overview: KG datasets and GNN tasks}
Our KG datasets include real KGs, such as MAG, YAGO, DBLP and WikiKG. The datasets are extracted from three very large KGs of different application domains: a general-fact KG (Yago\footnote{YAGO-4: \url{https://yago-knowledge.org/downloads/yago-4}}) and academic KGs (MAG\footnote{MAG-2020-05-29: \url{https://makg.org/rdf-dumps/}} and DBLP\footnote{DBLP versions March 2022 and Jan,March, and May 2023: \url{https://dblp.org/rdf/release/}}). These KGs contain 15.6 to 42.4 million vertices and up to 400 million triples. The number of node and edge types varies from 42 to 104 types. 
Existing SOTA methods for link prediction tasks on large KGs require excessive computing resources. Hence, we also used YAGO3-10\footnote{YAGO3-10: \url{https://paperswithcode.com/dataset/yago}}, a smaller version of YAGO.
Tables~\ref{tbl_exp_ds_Statistics} and~\ref{tbl_exp_tasks} summarize the details of the used KGs and the defined NC and LP tasks, respectively. 
Our benchmark will be available for further study~\footnote{More details of out benchmark is available in the supplementary materials \href{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/raw/KGTOSA_SupplementalMaterial.pdf}{\textcolor{blue}{here}}.}.\shorten 

We support two graph ML tasks on our benchmark datasets. The first task is the \textit{Node Classification (NC)} defined in \ref{def:NC}.
% as follows, for a $KG$ in definition \ref{def:kg} with $\mathcal{V}$ nodes and $\mathcal{R}$ relations. $\mathcal{A} \in \mathcal{R}^{|V|x|V|}$ represents the adjacency matrix, and $\mathcal{X} \in \mathcal{R}^{|\mathcal{V}|xF}$
% represents the node attribute matrix, where F is the number of features for each
% node. The goal is to train a GNN model that learns effective node representations $H$ to predict a label (class) for a set of nodes $ \subseteq \mathcal{V}$. KGs 
Unlike homogeneous datasets KGs may contain multi-label per node, In this study, we followed the SOTA works in \cite{OGB,SeHGNN,Shadow-GNN} and limit our tasks to single-label multi-class classification tasks.  In the case of multi-label associated with a single node, we choose the most frequent label as the node label. In that setting, we choose the accuracy metric to evaluate the task performance in addition to the training time and memory consumption. The train-valid-test splits are either split using a logical predicate that depends on the task or stratified random split with 80\% for training 10\% for validation and 10\% for testing. We provided two NC tasks per KG as in table \ref{tbl_exp_tasks}.

The second task is the \textit{Link Prediction (LP)} defined in \ref{def:LP}.
% as follows, for a $KG$ in definition \ref{def:kg} with $\mathcal{V}$ nodes and $\mathcal{R}$ relations the task is to train a GNN model that learns the existing facts structure and predict missing ones. The prediction should correctly infer a missing entity (object node) that completes the (s, p, ?o) triple where the $ type(s),type(?o) \in \mathcal{C}$ and $type(p) \in \mathcal{R}$. 
Large KGs usually contain a large number of \mathcal{R} relations that varies in their importance to a specific task,i.e., the \textit{is-a} edge is not of the same importance as discipline for an author-affiliation link prediction task. Large graphs require large training time and memory resources that can not be easily offered. We restrict our study to predict the missing objects for a target subject vertex and a single link type per task.  In that setting, we choose the Hits@10 metric to evaluate the task performance following SOTA in \cite{MorsE,OGB,Shadow-GNN} in addition to the training time and memory consumption. The train-valid-test splits are either split using 3 versions of the KG where the oldest version triples go for training, the newly added triples between the oldest and the middle version go for validation, and the newly added triples between the newest and the middle versions go for testing or splitting the KG per edge type randomly with 80\% for training 10\% for validation and 10\% for testing. We provide two LP tasks on DBLP-15M and YAGO3-10, one each.

 

% Similar to existing GNN benchmarks~\cite{OGB,OGB-LSC}, we used the accuracy metric for NC tasks and Hits@10 metric for LP tasks. None of the existing GNN benchmarks or systems used a KG of that scale and level of heterogeneity for node classification tasks, especially regarding the number of vertices and types of nodes and edges. 

% Existing benchmarks used handcrafted subgraphs of a KG, such as the MAG subgraph in open graph benchmark (OGBN-MAG)~\cite{OGB} with up to four node/edge types and less than 2 million vertices, or small heterogeneous graphs, as in Heterogeneous Graph Benchmark (HGB)~\cite{HGNN_Benchmark}, of thousands of vertices and a few types of nodes and edges.\shorten 

\input{tables/datasets_Staticstics.tex}
\input{tables/Tasks_Staticstics.tex}

% Existing GNN datasets are not suitable for evaluating our problem as they are either homogeneous graphs datasets as in \cite{OGB} or heterogeneous datasets extracted from real KGs as in \cite{OGB,HGNN_Benchmark} with small sizes and a few  numbers of node/edge types \cite{HGNN_Benchmark}. 

\subsection{Node Classification Datasets:}
\nsstitle{\textbf{MAG-42M 
 Paper-Venue (PV)}:} The dataset extracted from The MAG KG\cite{MAG} to train a GNN model that predicts the publication venue of a paper. The target nodes are papers and the prediction labels are their associated venues. The set of paper is the same set in OGBN-MAG \cite{OGB} dataset while including all neighbours nodes for a depth of 3 hops. The number of  classes (distinct venues) is 349. The training set includes papers published until 2018, the validation set includes papers published in 2019, and the test set includes papers published in 2020. the number of node types is 58, and the number of edge types is 62. The number of edges is 166M and the number of nodes is 42M, as shown in table \ref{tbl_exp_ds_Statistics}.\shorten

\nsstitle{\textbf{DBLP-15M 
 Paper-Venue (PV)}:} The dataset extracted from The DBLP KG\cite{KG_DBLP} to train a model that predicts the publication venue of a paper based on its publication history.  The target nodes are papers that have type \textit{(rec)} in KG, and the prediction labels are their associated venues, i.e., \textit{the  publishedIn edge}. Due to many distinct venues, we choose the top 50 frequent venues only, while any paper that does not belong to the top 50 is excluded. The training set includes papers published before 2020, the validation set includes papers published in 2020, and the test set includes papers published in 2021. The number of node types is 42 and the number of edge types is 48. The number of edges is 252M and the number of nodes is 15.6M.

\nsstitle{\textbf{MAG-42M 
 Paper-Discipline (PD)}:} The dataset extracted from The MAG KG\cite{MAG} to train a model that predicts the discipline of a paper based on its authors and citations.  The target nodes are papers, and the prediction labels are their associated disciplines. The set of paper is the same set in OGBN-MAG \cite{OGB} dataset while including all neighbours nodes for a depth of 3 hops.  Due to many distinct disciplines, we choose the top 50 frequent disciplines, while any paper that does not belong to the top 50 is excluded. The splitting criteria are the same as MAG-42M Paper-Venue (PV) dataset.

\nsstitle{\textbf{ DBLP-15M Author Affiliation-Country (AC):}} The dataset extracted from The DBLP KG\cite{KG_DBLP} to train a model that predicts the affiliation country of an author based on its collaboration history. The target nodes are authors that have type \textit{(person)} in KG and the prediction labels are their affiliation county i.e. \textit{(predicate type Affaliation\_Country)}.  Due to a large number of distinct countries, we choose the top 50 frequent countries only while any author affiliation that does not belong to the top 50 is excluded. The author nodes are randomly split for train-valid-test sets.\shorten
 
\nsstitle{\textbf{Yago4-30M KG (Place\-Country (PC))}:} The dataset extracted from The YAGO4 KG\cite{KG_Yago4} to train a model that predicts the country of a place based on its neighbour places.  
The target nodes are places that have type \textit{(place)} in KG and the prediction labels are their associated countries i.e. \textit{(predicate type locatedIn)}. Due to many distinct countries, we choose the top 200 frequent countries only while any place that does not belong to the top 200 is excluded. The places are randomly split for train-valid-test sets.\shorten

\nsstitle{\textbf{Yago-4 KG (Creative work\-Genre (CG))}:} 
The dataset extracted from The YAGO4 KG\cite{KG_Yago4} to train a model that predicts the genre of creative work.  
The target nodes are creative work-pieces that have type \textit{(genere)} in the KG and the prediction labels are their associated genres, i.e., \textit{(predicate type genre)}. Due to many distinct genres, we choose the top 51 frequent genres only, while any creative work that does not belong to the top 51 is excluded. The creative work nodes are randomly split for train-valid-test sets.\shorten


\subsection{Link Prediction Benchmark datasets:}
\nsstitle{\textbf{Yag03-10 Connected Airports (CA)}:} 
The dataset is extracted from The YAGO3 KG\cite{Yago3-10} for link prediction tasks. We train a model that predicts the missing \textit{isConnected} link between two nodes of type airport.  
The target nodes are airports that have \textit{isConnected} link in between in the KG. The \textit{isConnected} triples in the original validation and testing subsets are used for the validation and testing of the model. \shorten 

% The whole training triples are used for the training of the FG model While the {\sysName}$_{d_2h_1}$ BGP is used for the {\sysName} model.
\nsstitle{\textbf{ogbl-Wikikg2 Person Occupations (PO)}:}  The ogbl-wikikg2 \cite{OGB} dataset is extracted from the Wikidata knowledge base and it contains 2.5M entities and 535 edge types. The task is to predict the missing occupation links for a person (edge type P106). The dataset is split according to time with three versions of May, August, and November 2015 for training, validation and   testing, respectively. 

\nsstitle{\textbf{DBLP-15M Author Primary\-Affiliations (AA)}:} 
The dataset extracted from The DBLP KG\cite{KG_DBLP} versions Jan, March, and May 2023. The Jan version is used for the training. The model is trained to predict the missing \textit{research institute} nodes for a node of type author and \textit{Primary\-Affiliation} link. 
The target nodes are the author and research institute that have \textit{(Primary\-Affiliations)} link in between in the KG. \shorten

% The whole training triples are used for the training of the FG model While the {\sysName}$_{d_2h_1}$ BGP is used for the {\sysName} model.


==> sections/benchmark.tex <==
\section{Our KG Benchmark}
\label{sec:ben}

\input{tables/datasets_Staticstics.tex}

\subsection{An Overview: KG datasets and GNN tasks}
Our KG datasets include real KGs, such as MAG, DBLP, YAGO and WikiKG. The datasets are extracted from real KGs of different application domains: general-fact KGs (Yago~\footnote{YAGO-4: \url{https://yago-knowledge.org/downloads/yago-4}} and ogbl-wikikg2~\footnote{ogbl-wikikg2: \url{https://ogb.stanford.edu/docs/linkprop/\#ogbl-wikikg2}}) and academic KGs (MAG\footnote{MAG-2020-05-29: \url{https://makg.org/rdf-dumps/}} and DBLP~\footnote{DBLP versions March 2022 and Jan, March, and May 2023: \url{https://dblp.org/rdf/release/}}). These KGs contain up to 42.4 million vertices, 400 million triples, and tens to thousands of node/edge types. 
%
Existing HGNN methods for LP tasks on large KGs require excessive computing resources. Hence, we also used YAGO3-10~\footnote{YAGO3-10: \url{https://paperswithcode.com/dataset/yago}}, a smaller version of YAGO, and ogbl-wikikg2~\cite{OGB}, a dataset extracted from Wikidata. It contains 2.5M entities and 535 edge types.
Tables~\ref{tbl_exp_ds_Statistics} and~\ref{tbl_exp_tasks} summarize the details of the used KGs and our defined NC and LP tasks, respectively. 
Our benchmark will be available for further study.\shorten

%~\footnote{More details of out benchmark is available in the supplementary materials \href{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/raw/KGTOSA_SupplementalMaterial.pdf}{\textcolor{blue}{here}}.}.\shorten 

Our benchmark includes NC and LP tasks. In KGs, an NC task is categorized into single- or multi-label classifications, as defined in~\ref{def:NC}. Our benchmark followed existing benchmarks~\cite{OGB,SeHGNN,Shadow-GNN} and defined single-label NC tasks. We choose the accuracy metric for these NC tasks to evaluate the performance. The train-valid-test splits are either split using a logical predicate that depends on the task or stratified random split with 80\% for training, 10\% for validation and 10\% for testing. Table~\ref{tbl_exp_tasks} summarizes the details of the split schema and ratio. Our benchmark includes two NC tasks per KG.\shorten

For LP tasks, KGs contain many edge types that vary in importance to a specific task. For example, a user from an academic background will be interested in the predicates (edge type) \textit{discipline} and \textit{affiliation} in Wikidata but not in predicates related to movies and films. Moreover, training HGNNs for an LP task on a large KG of many edge types is computationally expensive. Hence, we define our LP tasks for a specific predicate to enable the HGNN methods to train the models with our available computing resources: a Linux machine with 32 cores and 3TB RAM. 
We choose the Hits@10 metric to evaluate the task performance following SOTA methods~\cite{MorsE,OGB,Shadow-GNN}. The train-valid-test splits are either split using three versions of the KG based on time or randomly. The details of the LP tasks are summarized in Table~\ref{tbl_exp_tasks}. 
%The oldest version is used for training, the middle version is used for validation, and the most recent version is used for testing. In some cases, we split the KG per edge type randomly with 80\% for training, 10\% for validation, and 10\% for testing. The details of the LP tasks are summarized in Table~\ref{tbl_exp_tasks}. 

\input{tables/Tasks_Staticstics.tex}

\subsection{Node Classification Datasets:}
\nsstitle{\textbf{MAG-42M 
Paper-Venue (PV)}:} The dataset extracted from The MAG KG\cite{MAG} to train a GNN model that predicts the publication venue of a paper. The target nodes are $736K$ papers, and the prediction labels are their associated venues. The set of paper is the same set in OGBN-MAG \cite{OGB} dataset while including all neighbours nodes for a depth of 3 hops. The number of classes (distinct venues) is $349$. The training set includes papers published until 2018, the validation set includes papers published in 2019, and the test set includes papers published in 2020. The number of node types is 58, and the number of edge types is 62. The number of edges is 166M, and the number of nodes is 42M, as shown in table \ref{tbl_exp_ds_Statistics}.\shorten

\nsstitle{\textbf{DBLP-15M Paper-Venue (PV)}:} The dataset extracted from DBLP~\cite{KG_DBLP} to train a model that predicts the publication venue of a paper. For the set of labels (distinct venues), we choose the top 50 frequent venues. Any paper that does not belong to the top 50 is excluded. This task includes $1.2M$ papers. The training set includes papers published before 2020, the validation set includes papers published in 2020, and the test set includes papers published in 2021.\shorten 

\nsstitle{\textbf{MAG-42M Paper-Discipline (PD)}:} The dataset extracted from MAG~\cite{MAG} to train a model that predicts the discipline of a paper based on its authors and citations. The target nodes are $710K$ papers, and the prediction labels are their associated disciplines. The set of paper is the same set in OGBN-MAG \cite{OGB} dataset while including all neighbours nodes for a depth of 3 hops. For the label set (distinct disciplines), we choose the top 50 frequent disciplines. We exclude any paper that does not belong to this set. The splitting criteria are the same as MAG-42M Paper-Venue (PV) dataset.

\nsstitle{\textbf{DBLP-15M Author Affiliation-Country (AC):}} The dataset extracted from the DBLP KG\cite{KG_DBLP} to train a model that predicts the affiliation country of an author based on its collaboration history. The target vertices are $92K$ authors with type \textit{(person)}. The label set includes the top 50 frequent countries. The author nodes are randomly split into train-valid-test sets.\shorten
 
\nsstitle{\textbf{Yago4-30M KG (Place\-Country (PC))}:} We used YAGO4~\cite{KG_Yago4} to train a model that predicts the country of a place based on its neighbour places. There are $734K$ target vertices of type \textit{(place)}. The label set includes the top 200 frequent countries. The places nodes are randomly split into train-valid-test sets.\shorten

\nsstitle{\textbf{Yago-4 KG (Creative-work Genre (CG))}:} 
We also used YAGO4~\cite{KG_Yago4} to train a model that predicts the genre of creative work. There are  $128K$ target vertices of type \textit{(Creative-Work)}. The label set includes the top 50 frequent genres. The creative work nodes are randomly split into train-valid-test sets.\shorten


\subsection{Link Prediction Benchmark datasets:}
\nsstitle{\textbf{Yag03-10 Connected Airports (CA)}:} 
We defined an LP task on YAGO3~\cite{Yago3-10} to predict the missing triples ⟨$v_t$,$p$,?⟩, where $v_t$ is of type airport and $p$ is the \textit{isConnected} predicate.  The \textit{isConnected} triples in the original validation and testing subsets are used for the validation and testing of the model.\shorten 

\nsstitle{\textbf{ogbl-Wikikg2 Person Occupations (PO)}:}  The ogbl-wikikg2 dataset is used for an LP task that predicts the missing occupation links for a person (edge type $P106$ in Wikidata). The dataset is split according to time with three versions of May, August, and November 2015 for training, validation and testing, respectively.

\nsstitle{\textbf{DBLP-15M Author Primary\-Affiliations (AA)}:} We defined another LP task on DBLP~\cite{KG_DBLP} to predict the missing triples ⟨$v_t$,$p$,?⟩, where $v_t$ is of type author and $p$ is the \textit{Primary\-Affiliation} predicate. Our training, validation, and test sets included the DBLP versions of Jan, March, and May 2023, respectively.


==> sections/introduction-MS-old.tex <==
\section{Introduction}
\label{sec:intro} 

A knowledge graph (KG) is a heterogeneous graph that includes nodes representing different entities ($\mathcal{V}$) of |$\mathcal{C}$| classes and edge types representing |$\mathcal{R}$| relations between these entities. $\mathcal{C}$ and $\mathcal{R}$ are the sets of node and edge types in the KG, respectively. Real-world KGs, such as Yago~\cite{KG_Yago4} and Wikidata \cite{KG_Wikidata}, have hundreds to thousands of node/edge types.
Graph neural networks (GNNs) have emerged as a powerful tool for analyzing KGs by defining real-world problems as node classification, such as recommender systems~\cite{gnnRS}, and entity alignment~\cite{gnnCrossLingual}, or link prediction, such as drug discovery~\cite{kgnn} and fraud detection~\cite{fraudDet} tasks.

Training GNNs on a large KG is computationally expensive and requires substantial memory to store and process the graph structures, associated features, and perform message-passing iterations~\cite{GraphSAINT, SeHGNN}. Some existing heterogeneous GNN methods~\cite{GraphSAINT, Shadow-GNN, FastGCN, MHGCN, MorsE} employ sampling and mini-batching training to reduce memory demands in training GNNs on large KGs by processing subsets of nodes or edges at a time. These methods help mitigate memory constraints while potentially sacrificing global context and long-range dependencies. Moreover, these methods utilize uniform sampling techniques over the whole KG. Hence, the complexity of the sampling method is dominated by the KG size and the sampled graphs may include nodes and edges that do not contribute to the training of a specific task~\cite{SeHGNN,HGNN_Benchmark}.\shorten 

\begin{figure}[t]
  \centering
  \includegraphics [width=\columnwidth]{figures/KGTOSA-Intro-Chart01-Accuracy.pdf}
  \vspace*{-7ex}
  \caption{(A) Accuracy (higher is better), (B) Training-Time (lower is better), (C) Training-Memory (lower is better). Training a node classification task ($T_{nc}$) to predict the paper venue using GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN} on a MAG graph with 42M vertices ($FG$). The handcrafted task-specific subgraph ($OGBN-MAG$) from $FG$ trades accuracy to reduce time and memory usage. {\sysName}'s task-specific subgraph is extracted automatically from $FG$ for $T_{nc}$ to optimize time and memory consumption while trying to improve accuracy.\shorten} 
  \vspace*{-2ex}
 \label{fig:motivation}  
\end{figure}

To overcome this limitation, AI practitioners manually handcraft a task-specific subgraph of a smaller $\mathcal{R}$ and $\mathcal{C}$ from a given KG for training GNNs~\cite{OGB,HGNN_Benchmark}. These handcrafted task-specific subgraphs (TSSG) help GNN methods alleviate the computation and memory cost of training ML tasks on large KGs. For example, the open graph benchmark (OGB)~\cite{OGB-LSC, OGB} provided OGBN-MAG, a subgraph of 21M triples out of 8.4B triples $\approx 0.2\%$ that is extracted from the Microsoft Academic Graph (MAG)~\cite{MAG} and is relevant to the node classification task for predicting a paper venue ($PV$). OGBN-MAG contains nodes and edges of only four types handcrafted by an AI practitioner for this specific task.
%
To demonstrate the effectiveness of this methodology, 
we trained the $PV$ task on a MAG graph of 166M triples with 42M vertices, 58 node types and 62 edge types; we refer to it as ($FG$). The $OGBN-MAG$~\cite{OGB} is a subgraph of $FG$ relevant to $PV$, i.e., task-specific subgraph for $PV$. 
In our training, we used the state-of-the-art GNN methods, namely GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN}. As shown in Figure~\ref{fig:motivation}, $OGBN-MAG$ trades the accuracy to help both methods reduce time and memory usage in training the task. Thus, the handcrafted task-specific subgraph is not optimized for achieving better accuracy than the accuracy of training the task on the full KG. Furthermore, generating the task-specific subgraphs demands a complete understanding of the task and the importance of each node and edge type in training the task. Thus, a handcrafted task-specific subgraph is time-consuming and challenging for AI practitioners.\shorten

This paper proposes different GNN meta-sampling approaches to address this problem and fully automate the extraction of TSSG from a given KG for a given task. Meta-sampling methods have been proposed in domains such as computer vision~\cite{PointCloudMetaSampling, Learning_to_Sample} and speech recognition~\cite{ASR_Meta_Sampling} to extract task-specific training datasets by integrating models with existing samplers. These methods have succeeded with homogenous datasets, e.g.,  images or text. Thus, we developed a GNN meta-sampling framework that formalizes three variations of GNN meta-sampling methods based on different methodologies. One of these methodologies is inspired by existing meta-sampling methods.
%
Overall, our results show that applying meta-sampling in training GNN tasks on KGs is challenging due to the significant heterogeneity present in KGs. Hence, a straightforward adaption of existing meta-sampling methods does not help alleviate the computation and memory cost of training GNNs on KGs. 

These results encouraged us to analyze these methodologies to identify graph patterns that correlate between a given task and the structure and properties of a KG. We developed {\sysName}, a SPARQL-based meta-sampling approach based on search queries leveraging built-in indices in RDF engines. Our {\sysName} extracts a TSSG automatically with negligible preprocessing overhead and  enables GNN methods to achieve substantial performance
gains in reducing time and memory usage while improving accuracy in most cases.
%
We integrated {\sysName} with the state-of-the-art (SOTA) GNN methods, namely SeHGNN~\cite{SeHGNN}, GraphSaint~\cite{GraphSAINT}, ShadowSAINT~\cite{Shadow-GNN}, and RGCN~\cite{RGCN}, and RDF engines, such as Virtuoso and Stardog. 
{\sysName} supports node classification  and link prediction tasks. Figure~\ref{fig:motivation} motivates the need for meta-sampling by showing the performance improvement in both GraphSAINT and SeHGNN using the task-specific subgraph extracted using {\sysName}. Our comprehensive evaluation using large real KGs and various ML tasks shows that {\sysName} enables GNN methods to converge faster and use less memory for training. Moreover, {\sysName} enables GNN methods to improve and achieve comparable levels of accuracy.\shorten 

In summary, our contributions are:
\begin{itemize}
\item our meta-sampling framework that formalizes different variations of GNN meta-sampling methods and analyzes their merits and demerits; (Section~\ref{sec:Meta-Sampling-Framework}).\shorten

\item pattern-based meta-sampling identifying graph patterns, which can be used as search queries to extract task-specific subgraphs from KGs for a given task; (Section~\ref{sec_subgraph-analysis}).\shorten

\item the first fully-fledged system ({\sysName}\footnote{
{\sysName} stands for KG \underline{T}ask \underline{O}riented \underline{Sa}mpling, and available at  \url{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/}}) for GNN meta-sampling. {\sysName} automates the entire pipeline of GNN training tasks on KGs built on top of existing RDF engines; (Section~\ref{sec:kg-tosa}).\shorten 

\item a comprehensive evaluation using our open KG benchmark (KGBen) and five GNN methods. KGBen includes four real KGs, six node classification tasks, and two link prediction tasks. The KGs have up to 40 million nodes and 400 million edges. {\sysName} achieves up to 70\% memory and time reduction while achieving significant accuracy improvement based on the KG size and the task; (Section~\ref{sec:expermients}).\shorten
\end{itemize}

% The remainder of this paper starts with Section~\ref{sec:background} to clarify the necessary background and ends with Section~\ref{sec:relatedwork} for related work and Section~\ref{sec:conclusion} for the conclusion.


% The remainder of this paper is organized as follows. Section~\ref{sec:background} clarifies the necessary background.  Section ~\ref{sec:Meta-Sampling-Framework} introduces our meta-sampling framework. Section~\ref{sec_subgraph-analysis} investigates the graph patterns of top-performing meta-sampling methods. Section~\ref{sec:kg-tosa} presents the {\sysName} system architecture. 
% % Section ~\ref{sec:benchmak} introduces our open KG  benchmark. 
% Section~\ref{sec:expermients} contains the experimental evaluation. Section~\ref{sec:relatedwork} discusses the related work, and Section~\ref{sec:conclusion} concludes the paper.\shorten

==> sections/introduction-TO3.tex <==

\section{Introduction}
\label{sec:intro} 

A knowledge graph (KG) is a heterogeneous graph that includes nodes representing different entities ($\mathcal{V}$) of |$\mathcal{C}$| classes, e.g., \textit{Paper} and \textit{Author} and edge types representing |$\mathcal{R}$| relations, e.g., \textit{publishedIn} and \textit{write}, between these entities. $\mathcal{C}$ and $\mathcal{R}$ are the sets of node and edge types in the KG, respectively. Real-world KGs, such as Yago~\cite{KG_Yago4} and Wikidata \cite{KG_Wikidata}, have hundreds to thousands of node/edge types.
Heterogeneous graph neural networks (HGNNs) have emerged as a powerful tool for analyzing KGs by defining real-world problems as node classification, such as recommender systems~\cite{gnnRS}, and entity alignment~\cite{gnnCrossLingual}, or link prediction, such as drug discovery~\cite{kgnn} and fraud detection~\cite{fraudDet} tasks.


% HGNN methods adopt mechanisms from GNNs for homogeneous graphs, such as multiple layers architecture and sampling in mini-batch training~\cite{GraphSAINT, Shadow-GNN, FastGCN, MHGCN, MorsE}.  The multiple layers architecture includes the utilization of multiple layers of graph convolutional networks (GCNs).In HGNN methods, the sampling mechanisms are originally proposed for homogeneous graphs. In mini-batching training, the adopted sampling approaches aim to sample a representative subset of nodes and edges (subgraph or batch) to learn overall a good representation of the KG~\cite{GraphSAINT}. Due to the KG heterogeneity, GNN tasks, such as node classification or link prediction tasks, target nodes of different types, where non-target nodes do not contribute evenly to training the task at hand. In HGNNs, the memory usage includes the graph structures, associated features, and multi-layer GCNs. The training time of HGNNs includes sampling in the case of mini-batch training and message-passing iterations~\cite{GraphSAINT, Shadow-GNN, SeHGNN}. Hence, training HGNNs on a large KG is computationally expensive and requires substantial memory and time~\cite{GraphSAINT, SeHGNN}, where the complexity~\footnote{The contribution of each factor to the complexity varies depending on the specific implementation, but these are the major factors in top-performing HGNN methods.} is influenced by the KG's size, density,  |$\mathcal{R}$|, and  |$\mathcal{C}$|~\cite{SeHGNN, GraphSAINT, Shadow-GNN}. 

HGNN methods adopt mechanisms from GNNs designed for homogeneous graphs, such as multi-layer graph convolutional networks (GCNs) and sampling in mini-batch training~\cite{GraphSAINT, Shadow-GNN, FastGCN, MHGCN, MorsE}.  
Unlike GNNs on homogeneous graphs, the number of GCN layers in HGNNs is associated with the number of edge types or metapaths in the heterogeneous graph to model the distinct relationships effectively. A metapath captures distinct semantic relationships (edge types) between node types. For example, the metapath Author-(write)-Paper-(publishedIn)-Venue (APV) describes the semantic relationships of an author who published a paper in a particular venue. 
In mini-batch HGNN training, the incorporated sampling mechanisms aim to obtain a subgraph (a subset of nodes or edges) that captures the representative structure of the original KG in general. The sampling is performed without considering node and edge types, where some specific types may have negligible or no effect in training a particular task. For example, a DBPedia~\footnote{The DBPedia KG contains information about movies and academic work.} subgraph, including instances of APV does not contribute to training a model predicting a movie genre. Hence, HGNN methods are not optimized for identifying subgraphs of a smaller subset of types to reduce the number of GCN layers in training a specific task. 

The space complexity of training HGNNs includes the memory required to store the graph structures, associated features, and multi-layer GCNs. Additionally, the time complexity includes the sampling process, in the case of mini-batch training, and the message-passing iterations needed to aggregate the embeddings of neighbouring nodes in each GCN.
That leads to computationally expensive memory usage and training time with large KGs, where the complexity~\footnote{The actual complexity varies depending on the specific implementation.} is influenced by the KG's size, density,  |$\mathcal{R}$|, and  |$\mathcal{C}$|~\cite{SeHGNN, GraphSAINT, Shadow-GNN}.
%
To alleviates the excessive computation on a large KG, AI practitioners manually handcraft a subgraph of a subset of $\mathcal{R}$ and $\mathcal{C}$ from a given KG for training HGNNs~\cite{OGB,HGNN_Benchmark}. We refer to this subgraph as a task-oriented subgraph (TOSG). Training the task using TOSG instead of the original KG helps HGNN methods reduce training time and memory usage. For example, the open graph benchmark (OGB)~\cite{OGB-LSC, OGB} provided OGBN-MAG, a subgraph of 21M triples out of 8.4B triples $\approx 0.2\%$ that is extracted from the Microsoft Academic Graph (MAG)~\cite{MAG} and is relevant to the node classification task for predicting a paper venue ($PV$). OGBN-MAG contains nodes and edges of only four types. 
% handcrafted by an AI practitioner for this specific task.

To demonstrate the effectiveness of this methodology, 
we trained the $PV$ task on a super-set of OGBN-MAG that contains 166M triples $\approx 2\%$ of MAG KG with 42M vertices, 58 node types and 62 edge types; we refer to it as ($MAG-42M$). The $OGBN-MAG$~\cite{OGB} is a subgraph of $MAG-42M$ relevant to $PV$, i.e., task-oriented subgraph for $PV$. 
%
We used the state-of-the-art GNN methods, namely GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN}. As shown in Figure~\ref{fig:motivation}, $OGBN-MAG$ trades the accuracy to help both methods reduce time and memory usage in training the task. 
Furthermore, crafting the TOSG demands a deep understanding of the KG's structure and the task's objectives. Hence, the TOSG extraction is a challenging and time-consuming process and does not guarantee to improve the model performance.  

This paper proposes {\sysName}~\footnote{
{\sysName} stands for KG \underline{T}ask \underline{O}riented \underline{Sa}mpling)}, an approach to automate the TOSG extraction for task-oriented HGNN training on a large KG. 
{\sysName} aims to discover a generic graph pattern that identifies a KG’s local and global structure related to a specific task. Hence, we develop task-oriented mechanisms sampling subgraphs specifically tailored to the requirements of a particular task. Our mechanisms start from the KG’s nodes, whose types are targeted by a given task, and expand to neighbouring nodes within $h$ hops. We adopt two expansion techniques: influenced-based and biased random walk sampling. Our influenced-based sampling utilizes a Personalized PageRank (PPR) score of nodes in the KG, where the PPR score is based on their relevance or importance to nodes of a particular type targeted by the task. Our biased random walk sampling performs random walks from nodes whose type is targeted by the task.\shorten  

We then conduct a thorough quality analysis of the subgraphs generated by our task-oriented sampling versus those generated by sampling methods adapted to top-performing HGNN methods. We defined assessment criteria for our comparative analysis under different categories, such as over-smoothing and data sufficiency. The over-smoothing criteria measure whether sampled subgraphs lead to indistinguishable node representations. The data sufficiency criteria measure the diversity of node/edge types in subgraphs to learn robust and generalizable patterns. Our comprehensive analysis leads to the discovery of a generic graph pattern that effectively captures the KG’s structure pertaining to a specific task. Our graph pattern preserves the local context by centralizing the sampling around nodes of types targeted by the task. Then, the graph pattern interlinks between the local context around each target node to generate a larger subgraph of node and edge types globally related to the task.

{\sysName} leverages our graph pattern to automate the extraction of a TOSG with negligible preprocessing overhead. We integrated {\sysName} with the state-of-the-art (SOTA) GNN methods, namely SeHGNN~\cite{SeHGNN}, GraphSaint~\cite{GraphSAINT}, ShadowSAINT~\cite{Shadow-GNN}, and RGCN~\cite{RGCN}, and RDF engines, such as Virtuoso and Stardog. Figure~\ref{fig:motivation} motivates the need for our {\sysName} approach by showing the performance improvement in both GraphSAINT and SeHGNN using the task-oriented subgraph extracted using {\sysName}.\shorten 

We have created a comprehensive benchmark comprising diverse, large-scale real KGs. Our benchmark encompasses KGs from the academic domain, such as the complete KG of MAG~\cite{MAG} and DBLP~\cite{KG_DBLP}, as well as 
two versions of YAGO as a general-purpose KG of different sizes, namely YAGO-4~\cite{KG_Yago4} and YAGO-3~\cite{Yago3-10}. We also have formulated various graph machine learning tasks, which have been translated into node classification and link prediction problems. Our benchmark includes KGs with a high degree of heterogeneity, featuring tens to hundreds of node and edge types. This high degree of heterogeneity presents challenging settings for SOTA HGNN methods. Our comprehensive evaluation using large real KGs and various ML tasks shows that {\sysName} enables GNN methods to converge faster and use less memory for training. Moreover, {\sysName} enables GNN methods to improve and achieve comparable levels of accuracy.\shorten  

\begin{figure}[t]
  \centering
  \includegraphics [width=\columnwidth]{figures/KGTOSA-Intro-Chart01-Accuracy.pdf}
  % \vspace*{-7ex}
  \caption{(A) Accuracy (higher is better), (B) Training-Time (lower is better), (C) Training-Memory (lower is better). Training a node classification task ($PV$) to predict the paper venue using ShaDowSAINT~\cite{Shadow-GNN} and SeHGNN ~\cite{SeHGNN} on a MAG graph with 42M vertices ($MAG-42M$). The handcrafted task-oriented subgraph ($OGBN-MAG$) from $MAG-42M$ trades accuracy to reduce time and memory usage. Our {\sysName}$_{d1h1}$ task-oriented subgraph is extracted automatically from $MAG-42M$ for $PV$ to reduce time and memory consumption while improving accuracy.\shorten} 
  % \vspace*{-2ex}
 \label{fig:motivation}  
\end{figure}

In summary, our contributions are:
\begin{itemize}

\item the first fully-fledged approach ({\sysName})~\footnote{available at \url{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/}} for task-oriented HGNN training based on our generic graph pattern identifying a KG's local and global context related to a specific task. {\sysName} utilizes this graph pattern to automatically extract the TOSG.\shorten 

\item two task-oriented sampling mechanisms used as baselines to analyze the quality of subgraphs sampled for a specific task versus subgraphs sampled using methods adapted in SOAT HGNN methods.     

\item a comprehensive evaluation using our KG benchmark and five SOTA GNN methods. Our KG benchmark includes four real KGs, six node classification tasks, and six link prediction tasks. The KGs have up to 42 million nodes and 400 million edges. {\sysName} achieves up to 70\% memory and time reduction while improving the model performance in terms of accuracy and inference time.\shorten
\end{itemize}


The remainder of this paper starts with Section~\ref{sec:background} to clarify the necessary background. Sections~\ref{sec:TOSampling} and~\ref{sec_approach} present our task-oriented sampling and the {\sysName} approach. Sections~\ref{sec:ben} and~\ref{sec:expermients} introduce our benchmark and evaluation. We highlights related work in Section~\ref{sec:relatedwork} and conclude the paper in Section~\ref{sec:conclusion}.

==> sections/introduction-old-TO1.tex <==

\section{Introduction}
\label{sec:intro} 

A knowledge graph (KG) is a heterogeneous graph that includes nodes representing different entities ($\mathcal{V}$) of |$\mathcal{C}$| classes, e.g., \textit{Paper} and \textit{Author} and edge types representing |$\mathcal{R}$| relations, e.g., \textit{publishedIn} and \textit{write}, between these entities. $\mathcal{C}$ and $\mathcal{R}$ are the sets of node and edge types in the KG, respectively. Real-world KGs, such as Yago~\cite{KG_Yago4} and Wikidata \cite{KG_Wikidata}, have hundreds to thousands of node/edge types.
Heterogeneous graph neural networks (HGNNs) have emerged as a powerful tool for analyzing KGs by defining real-world problems as node classification, such as recommender systems~\cite{gnnRS}, and entity alignment~\cite{gnnCrossLingual}, or link prediction, such as drug discovery~\cite{kgnn} and fraud detection~\cite{fraudDet} tasks.


Training HGNNs on a large KG is computationally expensive and requires substantial memory to store the graph structures and associated features and perform message-passing iterations~\cite{GraphSAINT, SeHGNN}. Some existing heterogeneous GNN methods~\cite{GraphSAINT, Shadow-GNN, FastGCN, MHGCN, MorsE} employ sampling and mini-batching training to reduce memory demands in training GNNs on large KGs by processing subsets of nodes or edges at a time. In mini-batching training, the adopted sampling approaches aim to sample a representative subset of nodes and edges (subgraph or batch) to learn overall a good representation of the KG~\cite{GraphSAINT}. Due to the KG heterogeneity, GNN tasks, such as node classification or link prediction tasks, target nodes of different types, where non-target nodes do not contribute evenly to training the task at hand. The adopted sampling approaches utilize uniform sampling techniques over the whole KG. Hence, they suffer two main limitations: \myNum{i} they do not consider a specific task, which leads to identifying subgraphs or batches, including nodes and edges, that do not contribute to the training of a particular task, and \myNum{ii} the complexity of the sampling method is dominated by the KG size and density ~\cite{SeHGNN,HGNN_Benchmark}. 
  
\begin{figure}[t]
  \centering
  \includegraphics [width=\columnwidth]{figures/KGTOSA-Intro-Chart01-Accuracy.pdf}
  \vspace*{-7ex}
  \caption{(A) Accuracy (higher is better), (B) Training-Time (lower is better), (C) Training-Memory (lower is better). Training a node classification task ($PV$) to predict the paper venue using ShaDowSAINT~\cite{Shadow-GNN} and SeHGNN ~\cite{SeHGNN} on a MAG graph with 42M vertices ($MAG-42M$). The handcrafted task-oriented subgraph ($OGBN-MAG$) from $MAG-42M$ trades accuracy to reduce time and memory usage. Our {\sysName}$_{d1h1}$ task-oriented subgraph is extracted automatically from $MAG-42M$ for $PV$ to reduce time and memory consumption while improving accuracy.\shorten} 
  \vspace*{-2ex}
 \label{fig:motivation}  
\end{figure}

To overcome these limitations, AI practitioners manually handcraft a task-oriented subgraph of a subset of $\mathcal{R}$ and $\mathcal{C}$ from a given KG for training GNNs~\cite{OGB,HGNN_Benchmark}. Using a handcrafted task-oriented subgraph (TOSG) instead of the full KG helps GNN methods alleviate the computation and memory cost of training ML tasks. For example, the open graph benchmark (OGB)~\cite{OGB-LSC, OGB} provided OGBN-MAG, a subgraph of 21M triples out of 8.4B triples $\approx 0.2\%$ that is extracted from the Microsoft Academic Graph (MAG)~\cite{MAG} and is relevant to the node classification task for predicting a paper venue ($PV$). OGBN-MAG contains nodes and edges of only four types handcrafted by an AI practitioner for this specific task.

To demonstrate the effectiveness of this methodology, 
we trained the $PV$ task on a super-set of OGBN-MAG that contains 166M triples $\approx 2\%$ of MAG KG with 42M vertices, 58 node types and 62 edge types; we refer to it as ($MAG-42M$). The $OGBN-MAG$~\cite{OGB} is a subgraph of $MAG-42M$ relevant to $PV$, i.e., task-oriented subgraph for $PV$. 
%
We used the state-of-the-art GNN methods, namely GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN}. As shown in Figure~\ref{fig:motivation}, $OGBN-MAG$ trades the accuracy to help both methods reduce time and memory usage in training the task. 
Furthermore, generating the task-oriented subgraphs demands a complete understanding of the task and the importance of each node and edge type in training the task. Thus, handcrafting a subgraph is time-consuming and challenging for AI practitioners.\shorten

This paper proposes {\sysName}\footnote{
{\sysName} stands for KG \underline{T}ask \underline{O}riented \underline{Sa}mpling)}, a graph-pattern-based approach to automatically extract a task-oriented subgraph (TOSG) from a KG for a given task. Our approach supports task-oriented GNN training on a TOSG. It identifies a generic graph pattern that helps extract a TOSG from a certain KG for a specific task to ignore nodes and edges that have negligible or no impact on training a GNN for a specific task. Hence, our graph-pattern approach will yield two main advantages: \myNum{i} the sampling method will extract from TOSG, i.e., instead of the full KG, subgraphs/batches that preserve the local and global context for a specific task, which helps a GNN method improve the modelling performance, e.g., accuracy or F1 score, for the task, and \myNum{ii} consume less training time and memory. We developed a SPARQL-based implementation of {\sysName} leveraging built-in indices in RDF engines to extract the TOSG automatically with negligible preprocessing overhead.

We developed a comparative framework to compare our \sysName{} to a wide range of baselines adapted from literature. In our framework, we analyzed the quality of sampled subgraphs with the proposed baselines against \sysName{}. Our study also considered two different sampling techniques adopted by existing HGNN methods. Our empirical analysis justifies the effectiveness and efficiency of our identified graph-pattern approach compared to existing sampling methods, which are task agnostic, and adapted baselines, which may improve model performance but cannot reduce memory and time required for training a GNN model, i.e., cannot scale to a large KG.\shorten

We have created a comprehensive benchmark comprising diverse, large-scale real KGs. Our benchmark encompasses KGs from the academic domain, such as the complete KG of MAG~\cite{MAG} and DBLP~\cite{KG_DBLP}, as well as 
two version of YAGO as a general-purpose KG of different sizes, namely YAGO-4~\cite{KG_Yago4} and YAGO-3~\cite{Yago3-10}. We also have formulated various graph machine learning tasks, which have been translated into node classification and link prediction problems using these KGs. Our benchmark includes KGs with a significant degree of heterogeneity, featuring tens to hundreds of node and edge types. The presence of such high heterogeneity within these large KGs presents a challenging scenario for state-of-the-art Graph Neural Network (GNN) methods.

We integrated {\sysName} with the state-of-the-art (SOTA) GNN methods, namely SeHGNN~\cite{SeHGNN}, GraphSaint~\cite{GraphSAINT}, ShadowSAINT~\cite{Shadow-GNN}, and RGCN~\cite{RGCN}, and RDF engines, such as Virtuoso and Stardog. Figure~\ref{fig:motivation} motivates the need for our {\sysName} approach by showing the performance improvement in both GraphSAINT and SeHGNN using the task-oriented subgraph extracted using {\sysName}. Our comprehensive evaluation using large real KGs and various ML tasks shows that {\sysName} enables GNN methods to converge faster and use less memory for training. Moreover, {\sysName} enables GNN methods to improve and achieve comparable levels of accuracy.\shorten 

In summary, our contributions are:
\begin{itemize}

\item the first fully-fledged approach~\footnote{available at \url{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/}} for task-oriented GNN training based on a graph pattern identifying a KG's local and global context related to a specific task; (Section~3). \shorten 

\item a comparative framework to analyze different baselines against our approach in supporting task-oriented GNN training. Our assessment shows our approach consumes negligible preprocessing overhead to extract a better-quality TOSG for training a specific task on a given KG; (Section~4).   

\item a comprehensive evaluation using our KG benchmark and five SOTA GNN methods. Our KG benchmark includes four real KGs, six node classification tasks, and six link prediction tasks; (Section~5). The KGs have up to 40 million nodes and 400 million edges. {\sysName} achieves up to 70\% memory and time reduction while achieving significant accuracy improvement based on the KG size and the task; (Section~\ref{sec:expermients}).\shorten
\end{itemize}

==> sections/introduction-old-TO2.tex <==

\section{Introduction}
\label{sec:intro} 

A knowledge graph (KG) is a heterogeneous graph that includes nodes representing different entities ($\mathcal{V}$) of |$\mathcal{C}$| classes, e.g., \textit{Paper} and \textit{Author} and edge types representing |$\mathcal{R}$| relations, e.g., \textit{publishedIn} and \textit{write}, between these entities. $\mathcal{C}$ and $\mathcal{R}$ are the sets of node and edge types in the KG, respectively. Real-world KGs, such as Yago~\cite{KG_Yago4} and Wikidata \cite{KG_Wikidata}, have hundreds to thousands of node/edge types.
Heterogeneous graph neural networks (HGNNs) have emerged as a powerful tool for analyzing KGs by defining real-world problems as node classification, such as recommender systems~\cite{gnnRS}, and entity alignment~\cite{gnnCrossLingual}, or link prediction, such as drug discovery~\cite{kgnn} and fraud detection~\cite{fraudDet} tasks.

HGNN methods adopt mechanisms from GNNs for homogeneous graphs, such as multiple layers architecture and sampling in mini-batch training~\cite{GraphSAINT, Shadow-GNN, FastGCN, MHGCN, MorsE}.  The multiple layers architecture includes the utilization of multiple layers of graph convolutional networks (GCNs), where the complexity~\footnote{The contribution of each factor to the complexity varies depending on the specific implementation, but these are the major factors in top-performing HGNN methods.} is influenced by the KG's size, density,  |$\mathcal{R}$|, and  |$\mathcal{C}$|~\cite{SeHGNN, GraphSAINT, Shadow-GNN}.
In HGNN methods, the sampling mechanisms are originally proposed for homogeneous graphs. Hence, these sampling mechanisms do not consider node and edge types. For example, the random walk mechanism adapted by GraphSAINT~\cite{GraphSAINT} samples nodes uniformly across the KG and traverses from the initial set of nodes by randomly selecting neighbouring nodes at each step. In Shadow-GNN~\cite{Shadow-GNN}, the sampling method calculates the importance of neighbouring nodes using the shortest path distance metric. However, these sampling mechanisms do not consider the node and edge types and samples for finding a representative subgraph in general, not for a specific task. 

Some HGNN methods use metapaths composed of high-level semantic relations, such as Author-(write)-Paper-(publishedIn)-Venue (APV) describing that an author published a paper in a particular venue. These methods sample instances of nodes and edges matching a certain metapath. The metapath-based HGNN methods consider the node and edge types. However, the sampling methods do not check the relevance of a certain metapath, e.g., APV, to a certain task. Hence, the incorporated sampling methods in HGNNs suffer two main limitations: \myNum{i} they do not consider a specific task, which leads to identifying subgraphs or batches, including nodes and edges, that do not contribute to the training of a particular task, and \myNum{ii} the complexity of the sampling method is dominated by the KG size and density ~\cite{SeHGNN,HGNN_Benchmark}. 
%
In HGNNs, the memory stores the graph structures, associated features, and multi-layer GCNs. The training time of HGNNs includes sampling in the case of mini-batch training and message-passing iterations~\cite{GraphSAINT, Shadow-GNN, SeHGNN}. Hence, training HGNNs on a large KG is computationally expensive and requires substantial memory and time~\cite{GraphSAINT, SeHGNN}. 

To alleviates the excessive computation, AI practitioners manually handcraft a task-oriented subgraph of a subset of $\mathcal{R}$ and $\mathcal{C}$ from a given KG for training HGNNs~\cite{OGB,HGNN_Benchmark}. Using the TOSG instead of the full KG helps GNN methods mitigate training time and memory usage of training ML tasks. For example, the open graph benchmark (OGB)~\cite{OGB-LSC, OGB} provided OGBN-MAG, a subgraph of 21M triples out of 8.4B triples $\approx 0.2\%$ that is extracted from the Microsoft Academic Graph (MAG)~\cite{MAG} and is relevant to the node classification task for predicting a paper venue ($PV$). OGBN-MAG contains nodes and edges of only four types handcrafted by an AI practitioner for this specific task.
%
To demonstrate the effectiveness of this methodology, 
we trained the $PV$ task on a super-set of OGBN-MAG that contains 166M triples $\approx 2\%$ of MAG KG with 42M vertices, 58 node types and 62 edge types; we refer to it as ($MAG-42M$). The $OGBN-MAG$~\cite{OGB} is a subgraph of $MAG-42M$ relevant to $PV$, i.e., task-oriented subgraph for $PV$. 
%
We used the state-of-the-art GNN methods, namely GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN}. As shown in Figure~\ref{fig:motivation}, $OGBN-MAG$ trades the accuracy to help both methods reduce time and memory usage in training the task. 
Furthermore, generating the task-oriented subgraphs demands a complete understanding of the task and the importance of each node and edge type in training the task. Thus, handcrafting a subgraph is time-consuming and challenging for AI practitioners.\shorten

This paper proposes {\sysName}\footnote{
{\sysName} stands for KG \underline{T}ask \underline{O}riented \underline{Sa}mpling)}, a graph-pattern-based approach to automatically extract a task-oriented subgraph (TOSG) from a KG for a given task. Our approach supports task-oriented GNN training on a TOSG. It identifies a generic graph pattern that helps extract a TOSG from a certain KG for a specific task to ignore nodes and edges that have negligible or no impact on training a GNN for a specific task. Hence, our graph-pattern approach will yield two main advantages: \myNum{i} the sampling method will extract from TOSG, i.e., instead of the full KG, subgraphs/batches that preserve the local and global context for a specific task, which helps a GNN method improve the modelling performance, e.g., accuracy or F1 score, for the task, and \myNum{ii} consume less training time and memory. We developed a SPARQL-based implementation of {\sysName} leveraging built-in indices in RDF engines to extract the TOSG automatically with negligible preprocessing overhead.

We developed a comparative framework to compare our \sysName{} to a wide range of baselines adapted from literature. In our framework, we analyzed the quality of sampled subgraphs with the proposed baselines against \sysName{}. Our study also considered two different sampling techniques adopted by existing HGNN methods. Our empirical analysis justifies the effectiveness and efficiency of our identified graph-pattern approach compared to existing sampling methods, which are task agnostic, and adapted baselines, which may improve model performance but cannot reduce memory and time required for training a GNN model, i.e., cannot scale to a large KG.\shorten

\begin{figure}[t]
  \centering
  \includegraphics [width=\columnwidth]{figures/KGTOSA-Intro-Chart01-Accuracy.pdf}
  \vspace*{-7ex}
  \caption{(A) Accuracy (higher is better), (B) Training-Time (lower is better), (C) Training-Memory (lower is better). Training a node classification task ($PV$) to predict the paper venue using ShaDowSAINT~\cite{Shadow-GNN} and SeHGNN ~\cite{SeHGNN} on a MAG graph with 42M vertices ($MAG-42M$). The handcrafted task-oriented subgraph ($OGBN-MAG$) from $MAG-42M$ trades accuracy to reduce time and memory usage. Our {\sysName}$_{d1h1}$ task-oriented subgraph is extracted automatically from $MAG-42M$ for $PV$ to reduce time and memory consumption while improving accuracy.\shorten} 
  \vspace*{-2ex}
 \label{fig:motivation}  
\end{figure}

We have created a comprehensive benchmark comprising diverse, large-scale real KGs. Our benchmark encompasses KGs from the academic domain, such as the complete KG of MAG~\cite{MAG} and DBLP~\cite{KG_DBLP}, as well as 
two version of YAGO as a general-purpose KG of different sizes, namely YAGO-4~\cite{KG_Yago4} and YAGO-3~\cite{Yago3-10}. We also have formulated various graph machine learning tasks, which have been translated into node classification and link prediction problems using these KGs. Our benchmark includes KGs with a significant degree of heterogeneity, featuring tens to hundreds of node and edge types. The presence of such high heterogeneity within these large KGs presents a challenging scenario for state-of-the-art Graph Neural Network (GNN) methods.

We integrated {\sysName} with the state-of-the-art (SOTA) GNN methods, namely SeHGNN~\cite{SeHGNN}, GraphSaint~\cite{GraphSAINT}, ShadowSAINT~\cite{Shadow-GNN}, and RGCN~\cite{RGCN}, and RDF engines, such as Virtuoso and Stardog. Figure~\ref{fig:motivation} motivates the need for our {\sysName} approach by showing the performance improvement in both GraphSAINT and SeHGNN using the task-oriented subgraph extracted using {\sysName}. Our comprehensive evaluation using large real KGs and various ML tasks shows that {\sysName} enables GNN methods to converge faster and use less memory for training. Moreover, {\sysName} enables GNN methods to improve and achieve comparable levels of accuracy.\shorten 

In summary, our contributions are:
\begin{itemize}

\item the first fully-fledged approach~\footnote{available at \url{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/}} for task-oriented GNN training based on a graph pattern identifying a KG's local and global context related to a specific task; (Section~3). \shorten 

\item a comparative framework to analyze different baselines against our approach in supporting task-oriented GNN training. Our assessment shows our approach consumes negligible preprocessing overhead to extract a better-quality TOSG for training a specific task on a given KG; (Section~4).   

\item a comprehensive evaluation using our KG benchmark and five SOTA GNN methods. Our KG benchmark includes four real KGs, six node classification tasks, and six link prediction tasks; (Section~5). The KGs have up to 40 million nodes and 400 million edges. {\sysName} achieves up to 70\% memory and time reduction while achieving significant accuracy improvement based on the KG size and the task; (Section~\ref{sec:expermients}).\shorten
\end{itemize}

==> sections/introduction-old-vldb.tex <==
\section{Introduction}
\label{sec:intro} 

A knowledge graph (KG) is a heterogeneous graph that includes nodes representing different entities ($\mathcal{V}$) of |$\mathcal{C}$| classes and edge types representing |$\mathcal{R}$| relations between these entities. $\mathcal{C}$ and $\mathcal{R}$ are the sets of node and edge types in the KG, respectively. Real-world KGs, such as Yago~\cite{KG_Yago4} and Wikidata \cite{KG_Wikidata}, have hundreds to thousands of node/edge types.
Graph neural networks (GNNs) have emerged as a powerful tool for analyzing KGs by defining real-world problems as node classification, such as recommender systems~\cite{gnnRS}, and entity alignment~\cite{gnnCrossLingual}, or link prediction, such as drug discovery~\cite{kgnn} and fraud detection~\cite{fraudDet} tasks.
Training GNNs on a large KG is computationally expensive due to the high computational complexity of the large graph convolutional networks (GCNs) processed for the KG~\cite{GraphSAINT, SeHGNN}. 
This process maintains multi-layer GCNs, whose complexity is proportional to the number of edge types~\cite{RGCN}, and has exponential growth with the number of nodes~\cite{SeHGNN, GraphSAINT, Graph-SAGE}.\shorten 

\begin{figure}[t]
  \centering
  \includegraphics [width=\columnwidth]{figures/KGTOSA-Intro-Chart01-Accuracy.pdf}
  \vspace*{-7ex}
  \caption{(A) Accuracy (higher is better), (B) Training-Time (lower is better), (C) Training-Memory (lower is better). Training a node classification task ($T_{nc}$) to predict the paper venue using GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN} on a MAG graph with 42M vertices ($FG$). The handcrafted task-specific subgraph ($OGBN-MAG$) from $FG$ trades accuracy to reduce time and memory usage. {\sysName}'s task-specific subgraph is extracted automatically from $FG$ for $T_{nc}$ to optimize time and memory consumption while trying to improve accuracy.\shorten} 
  \vspace*{-2ex}
 \label{fig:motivation}  
\end{figure}

Existing benchmarks for machine learning on graphs \cite{OGB,HGNN_Benchmark} adopt the task-specific subgraph methodology for training GNNs to alleviate the computation and memory cost of training ML tasks on real KGs. For example, the open graph benchmark (OGB)~\cite{OGB-LSC, OGB} provided OGBN-MAG, a subgraph of the Microsoft Academic Graph (MAG)~\cite{MAG} relevant to the node classification task for predicting a paper venue ($PV$). OGBN-MAG contains nodes and edges of only four types handcrafted by an AI practitioner for this specific task.\shorten 

To demonstrate the effectiveness of this methodology, 
we trained the $PV$ task on a MAG graph with 42M vertices, 58 node types and 62 edge types; we refer to it as ($FG$). The $OGBN-MAG$~\cite{OGB} is a subgraph of $FG$ relevant to $PV$, i.e., task-specific subgraph for $PV$. 
In our training, we used the state-of-the-art GNN methods, namely GraphSAINT~\cite{GraphSAINT} and SeHGNN ~\cite{SeHGNN}. As shown in Figure~\ref{fig:motivation}, $OGBN-MAG$ trades the accuracy to help both methods reduce time and memory usage in training the task. Thus, the handcrafted task-specific subgraph is not optimized for achieving better accuracy than the accuracy of training the task on the full KG. Furthermore, generating the task-specific subgraphs demands a complete understanding of the task and the effect of each node and edge type on training the task. Thus, a handcrafted task-specific subgraph is time-consuming and challenging for AI practitioners.\shorten
% with solid experience.\shorten

 Existing sampling-based GNN methods utilize uniform sampling techniques, which are not optimized to extract a task-specific subgraph for training a task on a KG. These methods can be categorized into: \myNum{i} heterogeneous GNN (HGNN), such as SeHGNN~\cite{SeHGNN}, MHGCN~\cite{MHGCN}, FastGTN~\cite{FastGTN} and  NARS~\cite{NARS}, and 
\myNum{ii} homogenous GNN methods adapted to heterogeneous graphs based on RGCN~\cite{RGCN}; we refer to them as RGCN-based methods. Examples of these methods are GraphSAINT~\cite{GraphSAINT}, Shadow-GNN~\cite{Shadow-GNN}, MorsE~\cite{MorsE}, and FastGCN~\cite{FastGCN}. 
HGNN methods attempt to improve the model's accuracy by proposing meta-path sampling techniques for heterogeneous graphs. These techniques help achieve slightly better accuracy than existing RGCN-based methods. However, the HGNN methods require a huge training time and memory usage, as stated in~\cite{SeHGNN,HGNN_Benchmark}. For example, SeHGNN~\cite{SeHGNN} with $FG$ improved the accuracy by 2\% but consumed 24\% extra memory and twice the time needed by GraphSAINT~\cite{GraphSAINT}, as shown in Figure~\ref{fig:motivation}. Hence, existing HGNN methods do not scale to a large KG. 
The RGCN-based GNN methods propose sampling techniques to avoid iterating over all vertices existing on a given graph~\cite{Shadow-GNN, MorsE, GraphSAINT, Graph-SAGE}. These techniques are not optimized to extract task-specific subgraphs.\shorten

Meta-sampling methods have been proposed in different application domains, such as computer vision~\cite{PointCloudMetaSampling, Learning_to_Sample} and speech recognition~\cite{ASR_Meta_Sampling}, to extract a task-specific training dataset. These methods proposed models to be integrated with the existing sampler to reduce the size of the sampled dataset. For instance, the meta-sampling in~\cite{Learning_to_Sample} predicts a rank for sampled 3D-shape points based on a given task and then trains a classification model based on the top-K points. These methods work with homogenous datasets, such as images or text. The KG GNN meta-sampling is challenging due to the high degree of heterogeneity in KGs. There is no meta-sampling method proposed for training GNN tasks on KGs. 

In this paper, we propose a GNN meta-sampling framework that formalizes three variations of GNN meta-sampling methods based on different methodologies. We analyzed these methodologies to identify graph patterns that correlate between a given task and the structure and properties of a KG. We developed {\sysName}, a SPARQL-based meta-sampling approach that is based on search queries leveraging built-in indices in RDF engines. We integrated {\sysName} with the state-of-the-art (SOTA) GNN methods, namely SeHGNN~\cite{SeHGNN}, GraphSaint~\cite{GraphSAINT}, ShadowSAINT~\cite{Shadow-GNN}, and RGCN~\cite{RGCN}, and RDF engines, such as Virtuoso and Stardog. \shorten
%
{\sysName} supports node classification  and link prediction tasks. Figure~\ref{fig:motivation} motivates the need for meta-sampling by showing the performance improvement in both GraphSAINT and SeHGNN using the task-specific subgraph extracted using {\sysName}. Our comprehensive evaluation using large real KGs and various ML tasks shows that {\sysName} enables GNN methods to converge faster and use less memory for training. Moreover, {\sysName} enables GNN methods to improve and achieve comparable levels of accuracy. In summary, our contributions are:
\begin{itemize}
\item our meta-sampling framework that formalizes different variations of GNN meta-sampling methods and analyzes their merits and demerits; (Section~\ref{sec:Meta-Sampling-Framework}).\shorten

\item pattern-based meta-sampling identifying graph patterns, which can be used as search queries to extract task-specific subgraphs from KGs for a given task; (Section~\ref{sec_subgraph-analysis}).\shorten

\item the first fully-fledged system ({\sysName}\footnote{
{\sysName} stands for KG \underline{T}ask \underline{O}riented \underline{Sa}mpling, and available at  \url{https://gitfront.io/r/CODS/LWYY16iUMSuE/KGTOSA/}}) for GNN meta-sampling. {\sysName} automates the entire pipeline of GNN training tasks on KGs built on top of existing RDF engines; (Section~\ref{sec:kg-tosa}).\shorten 

\item a comprehensive evaluation using our open KG benchmark (KGBen) and five GNN methods. KGBen includes four real KGs, six node classification tasks, and two link prediction tasks. The KGs have up to 40 million nodes and 400 million edges. {\sysName} achieves up to 70\% memory and time reduction while achieving significant accuracy improvement based on the KG size and the task; (Section~\ref{sec:expermients}).\shorten
\end{itemize}

% The remainder of this paper starts with Section~\ref{sec:background} to clarify the necessary background and ends with Section~\ref{sec:relatedwork} for related work and Section~\ref{sec:conclusion} for the conclusion.


% The remainder of this paper is organized as follows. Section~\ref{sec:background} clarifies the necessary background.  Section ~\ref{sec:Meta-Sampling-Framework} introduces our meta-sampling framework. Section~\ref{sec_subgraph-analysis} investigates the graph patterns of top-performing meta-sampling methods. Section~\ref{sec:kg-tosa} presents the {\sysName} system architecture. 
% % Section ~\ref{sec:benchmak} introduces our open KG  benchmark. 
% Section~\ref{sec:expermients} contains the experimental evaluation. Section~\ref{sec:relatedwork} discusses the related work, and Section~\ref{sec:conclusion} concludes the paper.\shorten

==> sections/subgraphs-analysis.tex <==
% \section{Quality Analysis and Graph Pattern}
 \section{The {\sysName} Approach}
\label{sec_approach}

This section analyzes the quality of subgraphs used in training GNN tasks, comparing those generated with and without meta-sampling methods. The goal is to identify graph patterns that link a KG with the vertices targeted by a GNN task, providing insights into the KG's structure and properties related to a specific task. Based on these graph patterns, meta-sampling could be performed as search queries on a KG.\shorten


\begin{figure*}[t]
\vspace*{-3ex}
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering        \includegraphics[width=\textwidth]{figures/YAGO-30M-RW.pdf}
         \caption{YAGO-30M (CreativeWork-Genere)}
         \label{fig:YAGO-30M-RW}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/MAG-42M-RW.pdf}
         \caption{MAG-42M (Paper-Venue)}
         \label{fig:MAG-42M-RW}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/DBLP-15M-RW.pdf}         
         \caption{DBLP-15M (Paper-Venue)}
         \label{fig:DBLP-15M-RW}
     \end{subfigure}
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/YAGO-30M-BRW.pdf}
         \caption{YAGO-30M (CreativeWork-Genere)}
         \label{fig:YAGO-30M-BRW}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/MAG-42M-BRW.pdf}
         \caption{MAG-42M (Paper-Venue)}
         \label{fig:MAG-42M-BRW}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{figures/DBLP-15M-BRW.pdf}
         \caption{DBLP-15M (Paper-Venue)}
         \label{fig:DBLP-15M-BRW}
     \end{subfigure}
     \vspace*{-4ex}
        \caption{ Each vertical pair of subgraphs are for the same GNN task on the same KG. The same colour means the same vertex or edge type per dataset.
        The upper subgraphs (a, b, and c) were generated by the random walk sampler in GraphSAINT (\textit{no meta-sampling}), while the lower subgraphs (d, e, and f) were generated using our biased random walk (BRW) meta-sampling. 
        Our meta-sampling biases the subgraphs towards target vertices for a given task, resulting in a higher ratio of target vertices connected to other extracted non-target vertices per subgraph. Node and edge types are color coded.\shorten}
        % The biased subgraphs (d), (e), and (f) correspond to uniformly sampled subgraphs (a), (b), and (c), respectively. 
\label{fig:subgraphQuality}
\end{figure*}



\subsection{Real KGs and GNN Tasks}
\label{sec:gqBench}

In our analysis, we employed three real KGs and performed four distinct node classification (NC) tasks. The first KG used was YAGO-30M, which contains over 30 million vertices and approximately 100 node/edge types. We conducted two NC tasks on YAGO-30M: \myNum{i} the CreativeWorks (CW) task, which predicts the genre of creative work, such as literature, painting, movie, or music, and \myNum{ii} the Place Country (PC) task, which predicts the country, where a given place is located. In both cases, we restricted the prediction to a limited set of categories; specifically, we focused on 51 genres for the CW task and 200 countries for the PC task. 
%
Moreover, we utilized two academic KGs: \myNum{i} MAG-42M, which contains over 42 million vertices and around 60 node/edge types, and \myNum{ii} DBLP-15M, which has over 15 million vertices and roughly 40 different node/edge types. On these KGs, we conducted a Paper-Venue task, which predicts the publication venue (e.g., AAAI, CDC, CVPR) for a given paper. We restricted the prediction to 50 venues in DBLP-15 and 350 venues in MAG-42M. It is worth noting that NC tasks become more challenging as the number of classes to predict increases.

\subsection{Quality of Subgraphs for A GNN Task}
\label{sec:QSub}

We investigated the quality of sampled subgraphs with and without meta-sampling using the KGs and GNN tasks highlighted in Section~\ref{sec:gqBench}. In our initial  investigation, we generated multiple subgraphs using random walk (RW) uniform sampling of the vanilla GraphSaint and our proposed GraphSaint+BRW method, described in Section~\ref{sec:brw}. GraphSaint+BRW outperformed GraphSaint as shown in Table 
 ~\ref{tbl:meta-samplers}. 
Each subgraph was sampled with $batch-size=20$ and $\textrm{\textit{walk-length }}h=2$, allowing the RW sampler to start from 20 initial vertices and expand up to two hops. These initial vertices were randomly selected in vanilla GraphSaint, while in GraphSaint+BRW, each initial vertex was a target vertex of the given task. Figure~\ref{fig:subgraphQuality} shows a pair of subgraphs per task/KG, where vertically, the upper subgraph is uniformly sampled, and the lower subgraph is a biased subgraph to the given task. 

% \textcolor{blue}{Meta-sampling is a technique used to guide GNN methods in accurately capturing relevant relations among variant vertices from a KG to achieve near-optimal performance for a specific task. This is achieved by identifying subgraphs of high quality that are task-specific, i.e., a subgraph of high quality for task $\mathcal{A}_i$ might not be of the same quality for task $\mathcal{A}_j$.}

In a GNN task, the method generates embeddings for a set of target vertices based on the captured graph structure from a KG during training. The embeddings of a target vertex $\mathcal{V}_T$ are obtained by aggregating the initial embeddings of $\mathcal{V}_T$ with those of its neighbouring vertices up to a specified hop distance $h$, where each iteration of aggregation reflects embeddings of neighbouring vertices at hop $h+1$ (e.g., neighbours of neighbours). The final embeddings of the target vertex are used in the learning process for the given task. Thus, our method generates task-specific subgraphs that are biased towards target vertices for a given task, resulting in a higher ratio of target vertices connected to other extracted vertices. This ensures there is enough data for learning for a specific task. 

\input{tables/table_biased_vs_unbiased_stat.tex}

Moreover, our task-specific subgraphs guarantee that non-target vertices are connected to at least one target vertex. 
Unlike task-specific subgraphs shown in Figures~\ref{fig:subgraphQuality}.d and ~\ref{fig:subgraphQuality}.e, the uniformly sampled subgraphs in Figures~\ref{fig:subgraphQuality}.a and ~\ref{fig:subgraphQuality}.b include a high ratio of disconnected non-target vertices from the target vertices.  
Disconnected vertices cannot contribute to the embeddings of the target vertices, as shown in Equation~\ref{eq_rgcn}. 
% These examples show how our meta-sampling captures relevant relations among variant vertices in a task-specific manner. Similar to BRW, we had similar results using our GA-FS method. For lack of space, we do not show them. 
%
Our task-specific subgraphs managed to: \myNum{i} reduce the average number of hops between non-target and target vertices, and \myNum{ii} identify a minimal set of edge types (features) reachable to the target vertices within less number of hops in average. For example, the subgraphs in Figures~\ref{fig:subgraphQuality}.c include (14, 15) (edge and node) types, which mostly describe non-target vertices in more than two hops from target vertices. 
Compared with the subgraphs in Figures~\ref{fig:subgraphQuality}.c, the one in Figures~\ref{fig:subgraphQuality}.f has only (9, 10) (edge, node) types primarily reachable in one hop. Hence, our meta-sampling helps reduces the size of $\mathcal{R}$ and $\mathcal{C}$ to avoid the over-smoothing problem discussed in Section~\ref{bg_GNN}.\shorten


\subsection{A Generic Graph Patterns for TOSGs}
Our observations on different KGs and tasks in Section~\ref{sec:QSub} show that the top-performing meta-sampling methods help extract subgraphs with \myNum{i} a sufficient number of target vertices ($\mathcal{V}_T$), \myNum{ii}  no vertices disconnected from $\mathcal{V}_T$, and \myNum{iii}  smaller sets of node and edge types. 
These three aspects are the main characteristics of high-quality graph patterns for task-specific subgraphs, which we refer to as \emph{target-centric graph pattern} (TCGP). This graph pattern extracts subgraphs centred around the target vertices within one or two hops. Restricting the number of hops is a heuristic to filter out less important node and edge types.
%
TCGP is optimized to achieve data sufficiency, include only task-relevant vertices and edges, and avoid over-smoothing. To verify that, we collected larger subgraphs than the ones used in Section~\ref{sec:QSub}. Thus, each subgraph was sampled with $batch-size=20,000$ and $\textrm{\textit{walk-length }}h=2$, i.e., the number of initial vertices is 20,000. This setting is used in training GNN tasks in different benchmarks~\cite{GraphSAINT, OGB}. We propose five metrics to measure these three indicators. 
The subgraphs have low variance among them. Hence, we limited our study to only ten extracted subgraphs per case and reported the average. Table~\ref{tab:tbl_YAGO_compare_stat} summarizes our results and reports the accuracy of the final trained model.\shorten  

\nsstitle{Data Sufficiency:} We measure data sufficiency using the ratio of target vertices (\emph{Target Vertices (\%)}) per subgraph. 
Across all tasks, the BRW method helps extract subgraphs of a higher percentage of target vertices, as shown in Table~\ref{tab:tbl_YAGO_compare_stat}. A subgraph of a lower percentage of target vertices provides insufficient training data. As noted in previous works, this negatively impacts the model's generalization and causes GNN overfitting, such as \cite{DropEdge} and \cite{GNN_Over_Smoothing}. 

\nsstitle{Task Relevance:}
A sampled subgraph, which includes a higher ratio of non-target vertices disconnected from target vertices (\emph{Target-Discon. (\%)}), does not help the learning process to be improved. They do not contribute to the model generalization, as shown in equation~\ref{eq_rgcn}. Hence, the subgraphs containing a high ratio of \emph{Target-Discon.} increase the training time and memory usage. 
BRW\footnote{BRW is implemented as an interleaving approach. Hence, the current results of BRW in Table~\ref{tbl:meta-samplers} do not show any time or memory reduction.} has zero percentage of \emph{Target-Discon} vertices, as shown in Table~\ref{tab:tbl_YAGO_compare_stat}.\shorten

\nsstitle{Over-Smoothing:}
We measure over-smoothing using three metrics, average distance from target vertices (\emph{Avg.Dist.Target}), the number of node types |$\mathcal{C}$|, and the number of edge types |$\mathcal{R}$|. 
Overall, BRW helps extract subgraphs of smaller \emph{Avg.Dist.Target} compared to the uniformly sampled subgraphs using RW. The structure and diversity of node/edge types in a KG can impact the reduction in the extracted $KG'$. In large KGs with a high degree of heterogeneity in node and edge types, the one-shot meta-sampling extracts a small $KG'$. Hence, it can reduce training time and memory. BRW may also enhance the model's performance, as shown in Table~\ref{tab:tbl_YAGO_compare_stat} with YAGO-30M and MAG-42M. For example, the subgraph extracted by BRW has the smallest $\mathcal{C}$ and $\mathcal{R}$ with YAGO and MAG. DBLP-15M has less degree of heterogeneity, e.g., the size of $\mathcal{C}$ and $\mathcal{R}$ is smaller than YAGO-30M and MAG-42M by almost 60\% and 33\%, respectively. Most of these types are related to the paper-venue task (PV). Hence, the RW sampler for PV/DBLP generates subgraphs where $\mathcal{C}$ and $\mathcal{R}$ are almost identical in size to the ones of BRW. Furthermore, these subgraphs of RW had no vertices disconnected from $\mathcal{V}_T$, resulting in a \emph{Target-Discon.(\%)} of zero. 

% Meta-sampling aims to optimize training and memory usage without compromising accuracy. For PV/DBLP, BRW achieves comparable accuracy to RW. 

% \nsstitle{One-shot Meta-sampling Based on Graph Patterns:}
% % Performing meta-sampling using BRW or GA-FS suffers different limitations. 
% BRW and GA-FS demand systems supporting random walk exploration (RWE) or genetic algorithms on a KG. Large KGs are widely stored in RDF engines, which have no support for both. It is very costly to migrate large KGs from these engines to existing frameworks that support RWE and graph traversal operations, such as Pytorch Geometric~\cite{pytorch-geometric} and DGL~\cite{DistDGL}. Most of these frameworks are memory-based approaches, which require colossal memory for large KGs. We have developed the KGNet system~\cite{KGNet}, which enables graph ML (GML) as a service on top of RDF engines. In KGNet, we aim to offload meta-sampling to RDF engines to provide memory-efficient GML support without migrating the full graph. We propose to perform one-shot meta-sampling as a search query against a certain KG to extract an initial $KG'$. This query is based on our TCGP.  The search queries should be supported efficiently by existing RDF engines. Unlike GA-FS, this variation of the one-shot meta-sampling can meet all our evaluation criteria discussed in Section~\ref{sec:Meta-Sampling-Framework}. 


% For example, there is a need to migrate these KGs outside RDF engines to use existing frameworks that support RWE and graph traversal operations, such as Pytorch Geometric~\cite{pytorch-geometric} and DGL~\cite{DistDGL}. Most of these frameworks are memory-based approaches, which require colossal memory for large KGs. We have developed the KGNet system~\cite{KGNet}, which enables graph ML (GML) as a service on top of RDF engines. In KGNet, we aim to offload meta-sampling to RDF engines to provide memory-efficient GML support without migrating the full graph. We propose to perform one-shot meta-sampling as a search query against a certain KG to extract an initial $KG'$. This query is based on our TCGP.  The search queries should be lightweight to reduce the meta-sampling cost. Unlike GA-FS, this variation of the one-shot meta-sampling can meet all our evaluation criteria discussed in Section~\ref{sec:Meta-Sampling-Framework}. 
% Full batch training GNN methods, such as RGCN, do not perform sampling, i.e., train a model on the full graph. The initial $KG'$ will help these methods significantly reduce memory usage, as initial $KG'$ is smaller than $KG$, especially in the case of a KG with a high degree of heterogeneity. 


==> tables/KGTOSA_MS_Cost_v0.tex <==

\begin{table}[t]
\vspace*{-3ex}
\caption{The preprocessing cost for GNN training on \myNum{i} a full graph (FG) migrated from RDF engine and \myNum{ii} KG' extracted using {\sysName}'s meta-sampling (MS) with $d=1$ and $h=1$.\shorten }
\vspace*{-1ex}
\label{tab:tbl_KGTOSA_preprocessing}
% \scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}&\multicolumn{2}{c|}{\textbf{KG Extra.}}& \multicolumn{2}{c|}{\textbf{Data Trans.}}& \multicolumn{2}{c|}{\textbf{\#Triples}} \\ 
&\multicolumn{2}{c|}{\textbf{Time (H)}}& \multicolumn{2}{c|}{\textbf{Time (H)}}& \multicolumn{2}{c|}{\textbf{ Millions}} \\ \hline
&FG Mig&MS&      
FG&$KG^\prime$&
FG&$KG'$\\ \hline
AC/DBLP-15M&2.6&0.05&0.14&0.01&95&2\\ \hline
PV/DBLP-15M&0.85&0.45&0.5&0.2&221&138\\ \hline
CG/YAGO-30M&6.5&1.5&1&0.1&24&1.2\\ \hline
PC/YAGO-30M&6.5&3&0.9&0.2&24&9.1\\ \hline
PV/MAG-42M&7.1&2.7&0.8&0.4&166&63\\ \hline
PD/MAG-42M&7&2.7&0.7&0.3&164&61\\ \hline
\end{tabular}
\end{table}


==> tables/Meta-Samplers.tex <==
\begin{table}[t]
\centering
\caption{
Our framework assessment for the proposed meta-sampling methods using DBLP\protect\footnotemark 
 and a node classification task predicting the paper venue. We integrated the methods with Graph-SAINT using TYPE-1 and TYPE-2 integration.\shorten}
\label{tbl:meta-samplers}
\begin{tabular} {lllll}
\toprule
Meta-Sampling & MS Cost &Training &Training & Accuracy\\
MS &Time (H) &Time (H) & Mem (GB) &\%\\\midrule
GraphSAINT&N/A &1.9 &46 &81.5 \\
\hline
GA-FS & 30.9 &\textbf{0.4} &\textbf{39}& \textbf{85.4} \\
VR-Model &2.75 &60.5 &51 &72.89 \\
BRW &\textbf{0} &2 &46 &82.23 \\
\bottomrule
\end{tabular}
\end{table}
\footnotetext{DBLP KG version is
\href{https://dblp.org/rdf/release/}{\textcolor{blue}{03-2022}}, we refer to it as DBLP15M in Section~\ref{sec:expermients}.}


% \begin{table}[t]
%  \caption{{\sysName}'s performance using different pre-trained models for training our QU and semantic affinity (SA) models. Our default settings using BART and fine-grained (FG) affinity achieve better F1 scores in most cases than the variations with GPT-3 in both QU and the coarse-grained (CG) affinity.\shorten
%  }
%  \label{tab:languagemodels}
%   \centering

%\begin{tabular}{lccc}
% \hline
%  \multicolumn{1}{c}{\textbf{}}& 
%  \multicolumn{1}{c}{\textbf{QU: BART}}&
%  \multicolumn{1}{c}{\textbf{QU: GPT-3}}&
%  \multicolumn{1}{c}{\textbf{QU: BART}}\\
%   \multicolumn{1}{c}{\textbf{Benchmarks}}& 
%  \multicolumn{1}{c}{\textbf{SA: FG}}&
%  \multicolumn{1}{c}{\textbf{SA: FG}}&
%  \multico\footnote{This experiment run on a cluster of 10 machines each machine contains 64 cores and 50GB of RAM.}lumn{1}{c}{\textbf{SA: GPT-3}}\\
% % \textbf{}&\textbf{BART + WE} & \textbf{GPT-3+WE} & \textbf{BART + GPT-3}\\
%         \hline
%         {\qald} & \textbf{43.99} & 41.00 & 41.85 \\
%         {\lcq} & 52.03 & \textbf{52.79} & 51.96\\
%         YAGO & \textbf{55.62} & 54.62 & 55.02 \\
%         DBLP & \textbf{54.78}  & 54.21 & 41.71\\ 
%         MAG &  \textbf{50.04} & 49.26 & 39.21\\ 
%         \hline
% \end{tabular}
% \end{table}

==> tables/NodeScoreFeatures.tex <==
\begin{table}[t]\centering
\caption{The set of features used to calculate the task-based node score. } \label{tbl_node_score}
\scriptsize
\begin{tabular}{|p{3em}|p{25em}|}
\toprule

Feature &Description 
\\\midrule
T &1 for target node and zero for non-target nodes \\
% \midrule
TI-H0 &How many in-going connections from target nodes at hops=0 \\
% \midrule
TO-H0 &How many out-going connections from target nodes at hops=0 \\
% \midrule
TI-H1 &How many in-going connections from target nodes at hops=1 \\
% \midrule
TO-H1 &How many out-going connections from target nodes at hops=1 \\
% \midrule
TI-H2 &How many in-going connections from target nodes at hops=2 \\
% \midrule
TO-H2 &How many out-going connections from target nodes at hops=2 \\
% \midrule
IC &How many in-going connections \\
% \midrule
OC &How many out-going connections \\
\bottomrule
\end{tabular}
\end{table}

==> tables/Tasks_Staticstics_old.tex <==
\begin{table}[t]
\vspace*{-1ex}
\centering
\caption{A summary of KGBen's tasks: Task Types (TT) are node classification (NC) or link prediction (LP), which predict a triple (s, p, o), where $type$($x$) is the type of s or o.}
\vspace*{-1ex}
\label{tbl_exp_tasks}
\begin{tabular}{lllll}\hline
TT&KG &( $type$(s), p, $type$(o)) \\\midrule
NC &MAG-42M &(Paper, publishedIn, \textbf{Venue}) \\
NC &MAG-42M&(Paper, discipline, \textbf{FieldOfStudy}) \\
NC &YAGO-30M&(CreativeWork, genre, \textbf{Genre})\\
NC &YAGO-30M&(Place, locatedIn, \textbf{Country})\\
% Person-Profession/LP &FB15K-237 &Profession &- &Random &MRR-Hits@10 \\
% Word Hyponym/LP &WN18 &Hyponym &- &Random &MRR-Hits@10 \\
NC &DBLP-15M&(Author, affiliation, \textbf{Country})\\
NC &DBLP-15M&(Publication, publishedIn,\textbf{Venue}) \\\midrule
LP &DBLP-15M &(Author, affiliatedWith, \textbf{Affiliation})\\
LP &YAGO3-10 &(Airport,connectTo,\textbf{Airport})\\ \midrule

% NC&OBGN-MAG&\textbf{Paper}/PublishedIn/Venue\\
% NC&DBLP-26K&\textbf{Author}/Discipline/FieldOfResearch\\
% NC&IMDB-12K&\textbf{Movie}/Type/Genres\\
% \bottomrule
\vspace*{-4ex}
\end{tabular}
\end{table}

% \begin{table*}[ht]\centering
% \centering
% \caption{The benchmark datasets statistics.}
% \label{tbl_exp_ds_Statistics}
% \scriptsize
% \begin{tabular}{|p{11em}|p{6em}|p{5em}|p{3em}|p{6em}|p{6em}|p{5em}|p{6em}|}
% % p{6em}|p{10em}|}
% \toprule
% Dataset & Abbreviation & KG & Task & \#FM Triples  & \# RS Triples  & \# SQ Triples & \# Node Types
% % &\# Edge Types& \# graph density  
% \\
% \midrule
% MAG Paper-Venue & MAG\_PV&MAG& NC  &NAN &21M &NA&NA
% % && 
% \\
% % \midrule
% MAG Paper-Discipline & MAG\_PD&MAG& NC&NAN& 21M&NA&NA
% % && 
% \\
% % \midrule
% DBLP Paper-Venue & DBLP\_PV &DBLP& NC&252M & 64M  &NA&NA
% % && 
% \\
% % \midrule
% DBLP Author-Country & DBLP\_AC&DBLP& NC &252M & 6M  &NA&NA
% % && 
% \\
% % \midrule
% Yago4 Place-Country & YAGO\_PC &Yago& NC&250M & NA  &NA&NA
% % && 
% \\
% % \midrule
% Yago4 Work-Category & YAGO\_WC&Yago& NC &250M & NA  &NA&NA
% % && 
% \\
% \midrule
% FB Person-Profession&FB15k\_PP&Free-Base& LP &237K& -  &NA&NA
% % && 
% \\
% % \midrule
% Yago10 Connected-Airport&YAGO10\_CA&Yago& LP &1.1M& -  &NA&NA
% % && 
% \\
% % \midrule
% WN Word-Hyponym&WN18\_WH&Word Net& LP &142K& -  &NA&NA
% % && 
% \\
% DBLP Author-Affiliation&DBLP\_AA&DBLP& LP &252M& -  &NA&NA
% % && 
% \\
% % Wiki Person-Occupations& Wikikg\_PO & Wikikg-v2 & LP &16.5M & NA &NA&NA& &\\
% \bottomrule
% \end{tabular}
% \end{table*}





==> tables/table01.tex <==
\begin{table}[t]\centering
\caption{ OGB datasets (sub-graphs) and their coverage ratio from the original KG.}\label{tbl_OGB_dataset}
\scriptsize
\begin{tabular}{|p{8em}|p{8em}|p{8em}|p{8em}|}
\toprule
ML Task &OGB Dataset (RS) &Original KG (FG) &Coverage Ratio
\\\midrule
\multirow{4}{*}{Node Classification}  &ogbn-products  &Amzon Product &66M/1B~= 6\% \\ 
% \cline{2-4}
&ogbn-mag &MAG &21M/8B~= 0.3\%  \\ 
% \cline{2-4}
&ogbn-arxiv &MAG &1.2M/8B~=0.01\% \\ 
% \cline{2-4}
&ogbn-papers-100M &MAG  &1.6B/8B~=20\% \\ 
% \cline{2-4}
\hline
\multirow{4}{*}{Link Prediction}   &ogbl-citation2  &MAG &30M/8B~= 0.4\% \\
 % \cline{2-4}
&ogbl-wikikg2 &WikiData &17M/3B~= 0.56\%  \\
% \cline{2-4}
&ogbl-ppa &STRING-DB v11 &30M/NA \\
% \cline{2-4}
&ogbl-ppa &BioKG  &30M/NA \\
% \cline{2-4}
\bottomrule
\end{tabular}
\end{table}

==> tables/table02.tex <==
\begin{table*}[!htp]\centering
\caption{GNN training pipeline steps including the role, techniques used, and challenges for each step}\label{tbl_GNN_pipeline}
\scriptsize
\begin{tabular}{|p{5em}|p{10em}|p{10em}|p{14em}|p{14em}|p{10em}|p{6em}|}
\toprule
\multirow{2}{} 
&\multirow{2}{50}{Graph Data Store} &\multicolumn{3}{c|}{Dataset ETL} &\multicolumn{2}{c|}{Graph ML} \\\cmidrule{3-7}
& &Dataset Extraction &Dataset Transformation & Dataloader &Training &Inferencing \\
\midrule
Role &Storing and maintaining graph data &Extract subgraph or a whole graph dataset & Automates dataset processing and splitting, to provide graph objects (vertices and relations) in adjacency matrix format &Load graph data into memory and convert it into sparse-matrics &Training GNN model &Predict nodes/edges \\
% \hline
Technique &Virtuoso, Jena,.. etc &KG Quering Languages i.e SPARQL, Cypher, etc. &Pandas data frames &Pytorch sparse matrix &full-graph or sample-based training. &Node classification Link prediction \\
% \hline
challenges &supporting machine learning on top of KG i.e providing ML learning operators on a form of SPARQL operators &retrieve graph dataset in a tabular format &Data format be compatible with PyTorch and its associated graph libraries i.e PyTorch Geometric \cite{PyGeometric}, and Deep Graph Library \cite{DistDGL} &Compressed sparse metrics that fit limited memory & better generalization and lower resources (Training time and memory) &Inductive Deductive \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table_GA.tex <==

\begin{table*}[]
\caption{Genetic Algorithm samples  statistics with random Walk sampler on DBLP.}
\label{tab:tbl_GA}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Indicator}            & \multicolumn{1}{l|}{}                              & \multicolumn{1}{c|}{\textbf{Data Sufficiency}}                  & \multicolumn{1}{c|}{\textbf{Task Relevance}}               & \multicolumn{3}{c|}{\textbf{Over-Smoothing}}                                                                                                                                                                                  & \multicolumn{2}{c|}{\textbf{Other Statistics}}                                                                     \\ \hline
\textbf{Task}              & \textbf{\# Nodes} & \textbf{Target Nodes (\%)}  & \textbf{Target-Disconnect.(\%)} & \textbf{Avg. Dist. to Target} &\textbf{\# Node Types}& \textbf{\# Edge Types} & \textbf{Accuracy (\%)}  &\textbf{Size (GB)}
% & Avg. $\delta$
\\ \hline
% CW/Genre(YAGO) & 50432   & 35.7     & 0  & 4.95                        & 34 & 33      & 36.72  & 2.6
% % & 4.23   
% \\ \hline
% Place/Country(YAGO)     & 56190   & 35.0   & 0   & 4.93                          & 25 & 24 & 89.52 & 3.2
% % & 2.67   
% \\ \hline
Paper/Venue(DBLP)     & 17156   & 41.7     & 1.92  & 3.9                      & 11 & 10   &85.4  & 14.9
% \\ \hline
% Paper/Venue(MAG)     & 56711   & 36.2     & 0 & 3.00                       & 26 & 25   & 81.08  & 6.4
% % & 6.4  
\\ \hline
\end{tabular}
\end{table*}



==> tables/table_KGTOSA_results.tex <==
\begin{table*}
\centering
\caption{KGTOSA-Samplers Results}\label{tab: }
\scriptsize
\begin{tabular}{|l|r|rrrrrr|rrrrrr|rrrrrrr|}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &\multirow{2}{*}{\textbf{Method}} &\multicolumn{6}{c}{\textbf{Accuracy(\%)}} &\multicolumn{6}{c}{\textbf{Training Time (Hours)}}&\multicolumn{6}{c}{\textbf{Training Memory (GB)}} \\\cmidrule{3-20}
& &\textbf{RS} &\textbf{FG} &\textbf{SQ} &\textbf{BS} &\textbf{PQ} &\textbf{BP} &\textbf{RS} &\textbf{FG} &\textbf{SQ} &\textbf{BS} &\textbf{PQ} &\textbf{BP} &\textbf{RS} &\textbf{FG} &\textbf{SQ} &\textbf{BS} &\textbf{PQ\_} &\textbf{BP} \\\midrule
\multirow{4}{*}{MAG\_PV} &GS &46.51 ± 0.47 &-1 & 82.50 ± 0.12 &82.35 ± 0.13 &-1 &-1 &0:58:29 &-1 &1:20:45 &1:34:17 &-1 &-1 &12 &-1 &13 &16.6 &-1 &-1 \\
&GS-Biased &47.55 ± 0.44 &-1 & 82.70 ± 0.12 &82.50 ± 0.10 &-1 &-1 &0:59:29 &-1 &1:22:45 &1:35:17 &-1 &-1 &12 &-1 &13 &16.6 &-1 &-1 \\
&RGCN & 36.79 ± 0.64 &-1 &78.08 ± 1.40 &80.23 ± 1.48 &-1 &-1 &0:09:10 &-1 &0:17:34 &0:18:30 &-1 &-1 &19 &-1 &19.7 &23.4 &-1 &-1 \\
&Shadow-SAINT &40.78 ± 0.15 &-1 &82.15 ± 0.55 &80.23 ± 1.48 &-1 &-1 &2:15:00 &-1 &5:10:14 &5:25:14 &-1 &-1 &12.8 &-1 &13.5 &16.9 &-1 &-1 \\
\midrule
\multirow{4}{*}{MAG\_PD} &GS &70.15 ± 0.54 &-1 &75.05 ± 0.09 &74.50 ± 0.32 &-1 &-1 &0:31:40 &-1 &1:08:30 &1:16:09 &-1 &-1 &11 &-1 &12.5 &13 &-1 &-1 \\
&GS-Biased & 70.34 ± 0.09 &-1 &75.68 ± 0.07 &75.19 ± 0.30 &-1 &-1 &0:32:40 &-1 &1:10:30 &1:17:09 &-1 &-1 &11 &-1 &12.5 &13 &-1 &-1 \\
&RGCN &68.83 ± 0.34 &-1 &72.33 ± 0.78 &73.08 ± 0.58 &-1 &-1 &0:07:00 &-1 &0:16:14 &0:16:44 &-1 &-1 &15.8 &-1 &19.2 &19.9 &-1 &-1 \\
&Shadow-SAINT &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 \\
\midrule
\multirow{4}{*}{DBLP\_PV} &GS &58.15 ± 0.14 & 81.79 ± 0.26 &89.88 ± 0.30 &90.42 ± 0.47 &90.85 ± 0.65 &89.98 ± 0.43 &0:15:23 &1:51:24 &1:25:15 &1:21:16 &1:40:54 &1:42:29 &9 &46.6 &36 &36.5 &41 &42.5 \\
&GS-Biased & 58.39 ± 0.29 &80.53 ± 1.37 &90.00 ± 1.47 &91.45 ± 0.58 &91.36 ± 0.99 & 90.28 ± 0.90 &0:17:23 &1:54:24 &1:27:48 &1:22:35 &1:41:23 &1:43:15 &9 &46.6 &36 &36.5 &41 &42.5 \\
&RGCN & 53.30 ± 1.15 &74.16 ± 0.87 &80.07 ± 1.25 &83.23 ± 2.03 &83.44 ± 3.64 &82.74 ± 2.61 &0:08:23 &1:58:10 &1:26:32 &1:24:42 &1:35:48 &1:37:18 &12.3 &220 &82 &82.6 &173 &175 \\
&Shadow-SAINT &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 \\
\midrule
\multirow{4}{*}{DBLP\_AC} &GS &33.08 ± 9.45 &80.79 ± 0.45 &78.88 ± 1.30 & 80.22 ± 0.12 &78.87 ± 0.59 &80.05 ± 0.36 &0:03:47 &2:49:34 &0:12:57 &0:23:00 &0:14:04 &0:27:38 &1.1 &79.8 &2.7 &11.4 &2.9 &13.2 \\
&GS-Biased & 33.05 ± 1.10 &85.07 ± 0.27 &79.26 ± 0.58 & 79.31 ± 0.86 &79.16 ± 0.32 &79.26 ± 0.54 &0:05:05 &2:57:00 &0:14:05 &0:28:57 &0:14:24 &0:33:32 &1.1 &79.8 &2.7 &11.4 &2.9 &13.2 \\
&RGCN & 40.90 ± 0.20 &75.86 ± 0.53 &66.07 ± 2.40 &66.80 ± 3.83 &61.59 ± 2.61 & 60.71 ± 0.70 &0:00:30 &2:13:46 &0:02:43 &0:04:14 &0:02:43 &0:08:54 &1.4 &207 &6 &16.7 &6.2 &26.7 \\
&Shadow-SAINT &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 &-1 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/table_KG_Statistics.tex <==

\begin{table}[t]
\centering
\caption{Statistics of real knowledge graphs.}
\label{tbl_KG_Statistics}
\scriptsize
\begin{tabular}{|p{8em}|p{3em}|p{3em}|p{6em}|p{6em}|p{4em}|}
\toprule
Knowledge Graph & \#Triples  & \#Entities  & \#Entity Types & \#Edge Types &  Size \\
\midrule
DBpedia \cite{KG_DBpedia} &4.7B &4.8M &2813&    8000&NA \\
% \midrule
Freebase \cite{Freebase_Google} &1.9B & 22M  &NA&NA&250 GB \\
% \midrule
\href{https://www.wikidata.org/wiki/Wikidata:Statistics}{Wikidata} \cite{KG_Wikidata} &3B &71M &\href{https://query.wikidata.org/#SELECT\%20\%20distinct\%20\%3FConcept\%0A\%20where\%20\%7B\%3Fs\%20a\%20\%3FConcept.\%7D\%20\%0Alimit\%2010000}{1301} & \href{https://www.wikidata.org/wiki/Wikidata:List_of_properties}{10,012} &440 GB \\
% \midrule
\href{https://yago-knowledge.org/downloads/yago-4}{Yago} \cite{KG_Yago4} &400M &50M&8902&156&40GB \\
% \midrule
\href{https://blog.dblp.org/2022/03/02/dblp-in-rdf}{DBLP} \cite{KG_DBLP} &252M &15.6M&42&47&35GB \\
% \midrule
\href{https://makg.org/}{MAG} \cite{MAG} &8B &610M&32&179 & \href{https://makg.org/rdf-dumps/}{1.2TB} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table_YAGO_FM_sample_stat.tex <==

\begin{table*}[]
\caption{ YAGO-4 and DBLP KG Sample Statistics with Random Walk Sampler.}
\label{tab:tbl_YAGO_FM_stat}
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Task               & \#Nodes & \% Target & Avg. Dist. & \% Disc. &\# Node Type & \# Edge Type & \% Acc. & Size \\ \hline
% & Avg. $\delta$
CW/Genre(YAGO) & 55720   & 1.1 \%      & 7.09                       & 76.6 \%    & 69 & 64      & 15.25 \% & 24.7 GB  \\ \hline
%   & 2.26 
Place/Country(YAGO)      & 55299   & 11.4 \%     & 7.46                       & 14.8 \%   & 85 & 80  & 79.28 \%  & 24.7 GB           \\ \hline
Paper/Venue(DBLP)      & 40618   & 29.94 \%     & 4.05                       & 0 \%  & 34 & 33 & 81.79 \%  & 40 GB           \\ \hline
Paper/Venue(MAG)     & 5724   & 2.03 \%     & 2.10                      & 69.1 \%  & 21 & 26 & 49.7 \%  & 35.8 GB  
\\ \hline
\end{tabular}
\end{table*}




% \begin{table}[]
% \caption{ YAGO-4 and DBLP KG Sample Statistics with Random Walk Sampler.}
% \label{tab:tbl_YAGO_FM_stat}
% \scriptsize
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Task            & \% Target &Avg. Target Deg. & Avg. Dist. & \% Disc.  & \% Acc. & Size \\ \hline
% % & Avg. $\delta$
% CW/Genre(YAGO) & 1.1 \%      & 2.26 & 7.09                       & 76.6 \%          & 15.25 \% & 24.7 GB  \\ \hline
% %   & 2.26 
% Place/Country(YAGO) & 11.4 \%   & 2.37  & 7.46                       & 14.8 \%   & 79.28 \%  & 24.7 GB           \\ \hline
% Paper/Venue(DBLP)      & 29.94 \%  & 5.71   & 4.05                       & 0 \%   & 81.79 \%  & 40 GB           \\ \hline
% Paper/Venue(MAG)     & 2.03 \%   &1.0  & 2.10                      & 69.1 \%   & 49.7 \%  & 35.8 GB  
% \\ \hline
% \end{tabular}
% \end{table}

==> tables/table_YAGO_biased_sample_stat.tex <==


\begin{table*}[]
\caption{ YAGO-4 and BDLP KG Sample Statistics with Biased Random Walk Sampler.}
\label{tab:tbl_YAGO_biased_stat}
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Task   & \# Nodes            & \%Target  & Avg. Dist. & \% Disc. &\# Node Type & \# Edge Type & \% Acc. 
& Size
% & Avg. $\delta$ 
\\ \hline
CW/Genre(YAGO) & 40936   & 61.2 \%      & 4.93                       & 0 \%  & 36  & 31      & 36.73 \%  & 24.7 GB\\ \hline
% & 2.44   

Place/Country(YAGO)      & 42016   & 55.3 \%     & 3.54                       & 0  \%     & 27  & 22      & 96.1 \%   & 24.7 GB\\ \hline
Paper/Venue(DBLP)      & 44886   & 65.37 \%     & 3.65                       & 0 \%  & 33  & 34    & 80.53 \%  & 40 GB             \\ \hline
Paper/Venue(MAG)     & 3991   & 99.5 \%     & 1.0                      & 0 \%  & 4  & 3    & 51.2\%  & 35 GB  
\\ \hline
\end{tabular}
\end{table*}



% \begin{table}[]
% \caption{ YAGO-4 and BDLP KG Sample Statistics with Biased Random Walk Sampler.}
% \label{tab:tbl_YAGO_biased_stat}
% \scriptsize
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Task          & \%Target  &Avg. Target Deg. & Avg. Dist. & \% Disc. & \% Acc. 
% & Size
% % & Avg. $\delta$ 
% \\ \hline
% CW/Genre(YAGO) &  61.2 \%   &2.44   & 4.93                       & 0 \%         & 36.73 \%  & 24.7 GB\\ \hline
% % & 2.44   

% Place/Country(YAGO)   & 55.3 \%   & 1.82  & 3.54                       & 0  \%         & 96.1 \%   & 24.7 GB\\ \hline
% Paper/Venue(DBLP)       & 65.37 \%  & 5.08  & 3.65                       & 0 \%   & 80.53 \%  & 40 GB             \\ \hline
% Paper/Venue(MAG)      & 99.5 \%  &1.0   & 1.0                      & 0 \%   & ?\%  & 35 GB  
% \\ \hline
% \end{tabular}
% \end{table}

==> tables/table_YAGO_star_sample_stat.tex <==

\begin{table}[t]
% \vspace*{-1ex}
\caption{
Statistics of subgraphs generated by {\sysName}$_{d1h1}$ for the same NC tasks considered in Table~\ref{tab:tbl_YAGO_compare_stat} for our BRW.}
\vspace*{-2ex}
\label{tab:tbl_KGTOSAStats}
% \scriptsize
\small
% \scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Indicator}            &  \textbf{Data Suff.}   & \textbf{Task Relevance} & \multicolumn{3}{c|}{\textbf{Over-Smoothing}}  \\ \hline
 \textbf{Task}& \textbf{$\mathcal{V}_T$(\%)} & \textbf{Target-Dis.(\%)}& \textbf{Avg.Dist} & \textbf{|$\mathcal{C}'$|} & \textbf{|$\mathcal{R}'$|}
 
%  \\\hline
% &\multicolumn{1}{c|}{BGP}      & BRW     & \multicolumn{1}{c|}{BGP}        & BRW        & \multicolumn{1}{c|}{BGP}         & BRW        & \multicolumn{1}{c|}{BGP}    & BRW   & \multicolumn{1}{c|}{BGP}    & BRW       
\\ \hline
CG/YAGO& 35.7&0&4.95&34&33  
% & 4.23   
\\ \hline
PC/YAGO &35.0&0&4.93&25& 24
% & 2.67   
\\ \hline
PV/DBLP&40.15&0&3.00&25&24 
\\ \hline
PV/MAG& 36.2& 0&3.00 & 26 &25  
% & 6.4  
\\ \hline
\end{tabular}
\vspace*{-4ex}
\end{table}


==> tables/table_YAGO_star_sample_stat_full.tex <==

\begin{table*}[t]
\caption{Statistics of {\sysName} (d=1, and h=1) sub-graphs vs BRW subgraphs with random walk sampler on Yago, DBLP, and MAG.\shorten}
\label{tab:tbl_YAGO_star_stat}
% \scriptsize
\small
% \scriptsize
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|c|}
\hline
\textbf{Indicator}            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{c|}{\textbf{Data Sufficiency}}                  & \multicolumn{2}{c|}{\textbf{Task Relevance}}               & \multicolumn{6}{c|}{\textbf{Over-Smoothing}}                                                                                                                                                                                  & \multicolumn{2}{c|}{\textbf{Other Statistics}}                                                                        \\ \hline
 \textbf{Task}          & \multicolumn{2}{c|}{\textbf{|$\mathcal{V}$|}} & \multicolumn{2}{c|}{\textbf{Target Vertices (\%)}} & \multicolumn{2}{c|}{\textbf{Target-Discon.(\%)}} & \multicolumn{2}{c|}{\textbf{Avg.Dist.Target}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{C}'$|}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{R}'$|}} & \multicolumn{2}{c|}{\textbf{Accuracy (\%) }}\\   \hline
           & \multicolumn{1}{c|}{BGP} & BRW & \multicolumn{1}{c|}{BGP}      & BRW     & \multicolumn{1}{c|}{BGP}        & BRW        & \multicolumn{1}{c|}{BGP}         & BRW        & \multicolumn{1}{c|}{BGP}    & BRW   & \multicolumn{1}{c|}{BGP}    & BRW   & \multicolumn{1}{c|}{BGP}    & BRW     \\ \hline
CG/YAGO& \multicolumn{1}{c|}{50432}&40936   &\multicolumn{1}{c|}{35.7}&   61.2  &\multicolumn{1}{c|}{ 0} &0 & \multicolumn{1}{c|}{4.95} &4.93                       & \multicolumn{1}{c|}{34}& 36& \multicolumn{1}{c|}{33}  &  31  & \multicolumn{1}{c|}{36.72} &36.73 
% & 4.23   
\\ \hline
PC/YAGO & \multicolumn{1}{c|}{56190} & 42016 & \multicolumn{1}{c|}{35.0}  &55.3 & \multicolumn{1}{c|}{0} & 0& \multicolumn{1}{c|}{4.93}&3.54                         & \multicolumn{1}{c|}{25} &27& \multicolumn{1}{c|}{24}&22 & \multicolumn{1}{c|}{89.52} &96.1
% & 2.67   
\\ \hline
PV/DBLP& \multicolumn{1}{c|}{51776}&44886 & \multicolumn{1}{c|}{40.15} & 65.37    &\multicolumn{1}{c|}{ 0} & 0& \multicolumn{1}{c|}{3.00} &3.56& \multicolumn{1}{c|}{25}& 33& \multicolumn{1}{c|}{24}  &34 & \multicolumn{1}{c|}{89.98} &80.53
\\ \hline
PV/MAG& \multicolumn{1}{c|}{56711}  & 44956& \multicolumn{1}{c|}{36.2}  & 78  & \multicolumn{1}{c|}{0}&0 &\multicolumn{1}{c|}{3.00} &2.99     & \multicolumn{1}{c|}{26} &20 &\multicolumn{1}{c|}{25}  &22 & \multicolumn{1}{c|}{81.08} &75.33
% & 6.4  
\\ \hline
\end{tabular}
\end{table*}


% \begin{table}[]
% \caption{Target-Centric Graph Pattern Samples Average Statistics with Random Walk Sampler on Yago-4, DBLP, and MAG KGs.}
% \label{tab:tbl_YAGO_star_stat}
% \scriptsize
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Task              & \% Target & Avg. Target Deg. & Avg. Dist. & \% Disc.  & \% Acc.  &Size
% % & Avg. $\delta$
% \\ \hline
% CW/Genre(YAGO)  & 35.7 \%     & 4.23 & 4.95                       & 0 \%          & 36.72 \%  & 2.6 GB
% % & 4.23   
% \\ \hline
% Place/Country(YAGO)   & 35.0 \% & 2.67   & 4.93                       & 0 \%   & 89.52 \%  & 3.2 GB
% % & 2.67   
% \\ \hline
% Paper/Venue(DBLP)  & 40.15 \%   & 7.75  & 3.00                       & 0 \%   & 89.98 \%  & 16.2 GB
% \\ \hline
% Paper/Venue(MAG)     & 52.5 \%  &7.67   & 3.12                      & 0 \%   & 82.5 \%  & 12 GB
% % & 2.67  
% \\ \hline
% \end{tabular}
% \end{table}

==> tables/table_biased_vs_unbiased_stat_v0.tex <==
\begin{table*}[t]
\caption{ Statistics of extracted subgraphs using URW, BRW, IBS, and $d_1h_1$ samplers on Yago-4, DBLP, and MAG KGs.}
% \vspace*{-3ex}
\label{tab:tbl_YAGO_compare_stat}
\small
% \scriptsize
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|c|}
\hline
\textbf{Indicator}            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{c|}{\textbf{Data Sufficiency}}   & \multicolumn{2}{c|}{\textbf{Task Relevance}}   & \multicolumn{6}{c|}{\textbf{Saving in Multi-layer GCNs}}                                                                                                                                                                                  & \multicolumn{2}{c|}{\textbf{Other Statistics}}                                                                        \\ \hline
 \textbf{Task}          & \multicolumn{2}{c|}{\textbf{|$\mathcal{V}$|}} & \multicolumn{2}{c|}{\textbf{$\mathcal{V}_T$ (\%)}} & \multicolumn{2}{c|}{\textbf{Target-Discon.(\%)}} & \multicolumn{2}{c|}{\textbf{Avg.Dist.Target}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{C}'$|}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{R}'$|}} & \multicolumn{2}{c|}{\textbf{Accuracy (\%) }}\\   \hline
& \multicolumn{1}{c|}{RW} & BRW & \multicolumn{1}{c|}{RW}      & BRW     & \multicolumn{1}{c|}{RW}        & BRW        & \multicolumn{1}{c|}{RW}         & BRW        & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW     \\ \hline
% & \multicolumn{1}{c|}{RW} & BRW & \multicolumn{1}{c|}{RW}      & BRW     & \multicolumn{1}{c|}{RW}        & BRW        & \multicolumn{1}{c|}{RW}         & BRW        & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & both  \\ \hline
CG/YAGO& \multicolumn{1}{c|}{55720}    & 40936  & \multicolumn{1}{c|}{1.1}           & 61.2       & \multicolumn{1}{c|}{76.6}            & 0             & \multicolumn{1}{c|}{7.09}             & 4.93          & \multicolumn{1}{c|}{69}          & 36       & \multicolumn{1}{c|}{64}          & 31       & \multicolumn{1}{c|}{15.25}       & 36.73    \\ \hline
PC/YAGO      & \multicolumn{1}{c|}{55299}    & 42016  & \multicolumn{1}{c|}{11.4}          & 55.3       & \multicolumn{1}{c|}{14.8}            & 0             & \multicolumn{1}{c|}{7.46}             & 3.54          & \multicolumn{1}{c|}{85}          & 27       & \multicolumn{1}{c|}{80}          & 22       & \multicolumn{1}{c|}{79.28}       & 96.1    \\ \hline
PV/DBLP  & \multicolumn{1}{c|}{40618}    & 44886  & \multicolumn{1}{c|}{29.94}         & 65.37      & \multicolumn{1}{c|}{0}               & 0             & \multicolumn{1}{c|}{4.05}             & 3.65          & \multicolumn{1}{c|}{34}          & 33       & \multicolumn{1}{c|}{33}          & 34       & \multicolumn{1}{c|}{81.79}       & 80.53      \\ \hline
PV/MAG   & \multicolumn{1}{c|}{36149}     & 44956   & \multicolumn{1}{c|}{4.90}          & 78.0       & \multicolumn{1}{c|}{89.27}            & 0             & \multicolumn{1}{c|}{3.00}              & 2.99           & \multicolumn{1}{c|}{48}          & 20        & \multicolumn{1}{c|}{43}          & 22        & \multicolumn{1}{c|}{73.79 }   &   75.33 \\ \hline
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multicolumn{1}{c|}{IBS} & $d_1h_1$ & \multicolumn{1}{c|}{IBS}      & $d_1h_1$     & \multicolumn{1}{c|}{IBS}        & $d_1h_1$        & \multicolumn{1}{c|}{IBS}         & $d_1h_1$        & \multicolumn{1}{c|}{IBS}    & $d_1h_1$   & \multicolumn{1}{c|}{IBS}    & $d_1h_1$   & \multicolumn{1}{c|}{IBS}    & $d_1h_1$     \\ \hline
           % & \multicolumn{1}{c|}{RW} & BRW & \multicolumn{1}{c|}{RW}      & BRW     & \multicolumn{1}{c|}{RW}        & BRW        & \multicolumn{1}{c|}{RW}         & BRW        & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & both  \\ \hline
CG/YAGO& \multicolumn{1}{c|}{78562}    & 50429.2  & 
\multicolumn{1}{c|}{82.4}& 35.7 &
\multicolumn{1}{c|}{0}& 0 & 
\multicolumn{1}{c|}{6.8}& 4.95& 
\multicolumn{1}{c|}{33}& 34& 
\multicolumn{1}{c|}{33}& 33&
\multicolumn{1}{c|}{42}&36.72 \\ \hline
PC/YAGO      & \multicolumn{1}{c|}{}    &   & \multicolumn{1}{c|}{}& 35.0&
\multicolumn{1}{c|}{0}& 0& 
\multicolumn{1}{c|}{}& 4.93& 
\multicolumn{1}{c|}{}& 25& 
\multicolumn{1}{c|}{}& 24&
\multicolumn{1}{c|}{97.2}&89.52 \\ \hline
PV/DBLP  & \multicolumn{1}{c|}{128026}& 51833.3 & 
\multicolumn{1}{c|}{19.4}& 40.15&
\multicolumn{1}{c|}{0}& 0& 
\multicolumn{1}{c|}{}& 3.00& 
\multicolumn{1}{c|}{32}& 24& 
\multicolumn{1}{c|}{33}& 25&
\multicolumn{1}{c|}{85.4}&89.88 \\ \hline
PV/MAG   & \multicolumn{1}{c|}{92103.4} &56744.8 & 
\multicolumn{1}{c|}{26.5}& 36.2&
\multicolumn{1}{c|}{0}& 0& 
\multicolumn{1}{c|}{}& 3.00& 
\multicolumn{1}{c|}{23}& 26& 
\multicolumn{1}{c|}{29}& 25&
\multicolumn{1}{c|}{75.4}&81.08 \\ \hline
\end{tabular}
\end{table*}

==> tables/table_biased_vs_unbiased_stat_v1.tex <==
\begin{table*}[t]
\centering
\vspace*{-3ex}
\caption{ Statistics of extracted subgraphs using URW, BRW, IBS, and {\sysName}$_{d_1h_1}$ on Yago-4, DBLP, and MAG KGs. Our SPARQL-based method using $_{d_1h_1}$ achieves similar statistics and comparable accuracy to BRW and IBS. However, BRW and IBS consume excessive computing resources w.r.t the SPARQL-based method as shown in Figure~\ref{fig:DifferentParameters}.}
\vspace*{0ex}
\label{tab:tbl_YAGO_compare_stat}
% \small
\scriptsize
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|cc|c|}
\hline
\textbf{Indicator} & \multicolumn{4}{c|}{$|\textbf{KG}^{\prime}|$}& \multicolumn{12}{c|}{\textbf{Data Sufficiency}} \\ \hline
 \textbf{Task}& \multicolumn{4}{c|}{$|\textbf{\mathcal{V}}|$} & \multicolumn{4}{c|}{\textbf{$\mathcal{V}_T$ (\%)}} & \multicolumn{4}{c|}{$|\textbf{\mathcal{C}'}|$} & \multicolumn{4}{c|}{$|\textbf{\mathcal{R}'}|$}
\\\hline
&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}
\\ \hline
CG/YAGO& \multicolumn{1}{c|}{55720}& 40936  & \multicolumn{1}{c|}{\textbf{78562}}&50429& \multicolumn{1}{c|}{1.1}&61.2& \multicolumn{1}{c|}{\textbf{82.4}}& 35.7& \multicolumn{1}{c|}{\textbf{69}}& \multicolumn{1}{c|}{36}& \multicolumn{1}{c|}{33}& \multicolumn{1}{c|}{34}&\multicolumn{1}{c|}{\textbf{64}}&\multicolumn{1}{c|}{31}&\multicolumn{1}{c|}{33}&    \multicolumn{1}{c|}{33}\\ \hline
PC/YAGO      & \multicolumn{1}{c|}{55299}    & 42016  & \multicolumn{1}{c|}{\textbf{79830}}          &50419& \multicolumn{1}{c|}{11.4}&55.3 & \multicolumn{1}{c|}{\textbf{74.6}}&35& \multicolumn{1}{c|}{\textbf{85}}&27&\multicolumn{1}{c|}{41}&25&\multicolumn{1}{c|}{\textbf{80}}&22& \multicolumn{1}{c|}{39}&\multicolumn{1}{c|}{24}\\ \hline
PV/DBLP  & \multicolumn{1}{c|}{40618}    & 44886  & \multicolumn{1}{c|}{\textbf{128026}}         & 51833      & \multicolumn{1}{c|}{29.9}& \textbf{65.4}& \multicolumn{1}{c|}{19.4}&40.2&\multicolumn{1}{c|}{\textbf{34}}&33& \multicolumn{1}{c|}{32}&24& \multicolumn{1}{c|}{33}&\textbf{34}& \multicolumn{1}{c|}{33}&\multicolumn{1}{c|}{25}\\ \hline
PV/MAG   & \multicolumn{1}{c|}{\36149}     & 44956   & \multicolumn{1}{c|}{\textbf{92103}}          & 56744       & \multicolumn{1}{c|}{4.9}&\textbf{78}& \multicolumn{1}{c|}{26.5}& 36.2&\multicolumn{1}{c|}{\textbf{48}}& 20& \multicolumn{1}{c|}{23}& 26& \multicolumn{1}{c|}{\textbf{34} }   &22 & \multicolumn{1}{c|}{29}&\multicolumn{1}{c|}{25}\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Indicator} & \multicolumn{12}{c|}{\textbf{Graph Topology}}& \multicolumn{4}{c|}{\textbf{Other Statistics}} \\ \hline
 \textbf{Task}& \multicolumn{4}{c|}{\textbf{Target-Discon.(\%)}} & \multicolumn{4}{c|}{\textbf{Avg.Dist.Target}} & \multicolumn{4}{c|}{\textbf{Max.Dist.Target}} & \multicolumn{4}{c|}{\textbf{Accuracy}}
\\\hline
&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}&\multicolumn{1}{c|}{RW} & \multicolumn{1}{c|}{BRW}&\multicolumn{1}{c|}{IBS}&\multicolumn{1}{c|}{$d_1h_1$}
\\ \hline

CG/YAGO& \multicolumn{1}{c|}{\textbf{76.7}}    & 0  & 
\multicolumn{1}{c|}{0}&0&
\multicolumn{1}{c|}{\textbf{7.1}}& 4.23 & 
\multicolumn{1}{c|}{4.7}& 4.18& 
\multicolumn{1}{c|}{\textbf{8}}&5& 
\multicolumn{1}{c|}{6}&5&
\multicolumn{1}{c|}{15.25}&36.73 & \multicolumn{1}{c|}{\textbf{42}}&    \multicolumn{1}{c|}{36.72} \\ \hline
PC/YAGO & \multicolumn{1}{c|}{14.8}&0& \multicolumn{1}{c|}{0}&0&
\multicolumn{1}{c|}{\textbf{7.46}}&4.12& 
\multicolumn{1}{c|}{5.2}&4.62& 
\multicolumn{1}{c|}{\textbf{8}}&5& 
\multicolumn{1}{c|}{6}&5&
\multicolumn{1}{c|}{79.28}&96.1 & \multicolumn{1}{c|}{\textbf{97.2}}&    \multicolumn{1}{c|}{89.52} \\ \hline
PV/DBLP  & \multicolumn{1}{c|}{0}& 0 & 
\multicolumn{1}{c|}{0}&0&
\multicolumn{1}{c|}{\textbf{4.23}}&3.71& 
\multicolumn{1}{c|}{3.95}&3.1& 
\multicolumn{1}{c|}{\textbf{5}}&4& 
\multicolumn{1}{c|}{\textbf{5}}&4&
\multicolumn{1}{c|}{81.79}&80.53 & \multicolumn{1}{c|}{85.4}&    \multicolumn{1}{c|}{\textbf{89.52}} \\ \hline
PV/MAG   & \multicolumn{1}{c|}{\textbf{89.3}} &0& 
\multicolumn{1}{c|}{0}&0&
\multicolumn{1}{c|}{3.1}& 2.9& 
\multicolumn{1}{c|}{\textbf{3.2}}& 3.00& 
\multicolumn{1}{c|}{\textbf{4}}&3& 
\multicolumn{1}{c|}{\textbf{4}}&3&    \multicolumn{1}{c|}{73.79}&75.33&
\multicolumn{1}{c|}{75.4}&\textbf{81.08} \\ \hline
\end{tabular}
% \vspace*{-3ex}
\end{table*}



==> tables/table_quality_TOsampling.tex <==
\begin{table*}[t]
\caption{ Statistics for RW and BRW random walk samplers on Yago-4, DBLP, and MAG KGs.}
\vspace*{-3ex}
\label{tab:tbl_YAGO_compare_stat}
\small
% \scriptsize
\begin{tabular}{|c|cc|cc|cc|cc|cc|cc|cc|c|}
\hline
\textbf{Indicator}            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{c|}{\textbf{Data Sufficiency}}                  & \multicolumn{2}{c|}{\textbf{Task Relevance}}               & \multicolumn{6}{c|}{\textbf{Over-Smoothing}}                                                                                                                                                                                  & \multicolumn{2}{c|}{\textbf{Other Statistics}}                                                                        \\ \hline
 \textbf{Task}          & \multicolumn{2}{c|}{\textbf{|$\mathcal{V}$|}} & \multicolumn{2}{c|}{\textbf{$\mathcal{V}_T$ (\%)}} & \multicolumn{2}{c|}{\textbf{Target-Discon.(\%)}} & \multicolumn{2}{c|}{\textbf{Avg.Dist.Target}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{C}'$|}} & \multicolumn{2}{c|}{\textbf{|$\mathcal{R}'$|}} & \multicolumn{2}{c|}{\textbf{Accuracy (\%) }}\\   \hline
           & \multicolumn{1}{c|}{RW} & BRW & \multicolumn{1}{c|}{RW}      & BRW     & \multicolumn{1}{c|}{RW}        & BRW        & \multicolumn{1}{c|}{RW}         & BRW        & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW     \\ \hline
           % & \multicolumn{1}{c|}{RW} & BRW & \multicolumn{1}{c|}{RW}      & BRW     & \multicolumn{1}{c|}{RW}        & BRW        & \multicolumn{1}{c|}{RW}         & BRW        & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & \multicolumn{1}{c|}{RW}    & BRW   & both  \\ \hline
CG/YAGO& \multicolumn{1}{c|}{55720}    & 40936  & \multicolumn{1}{c|}{1.1}           & 61.2       & \multicolumn{1}{c|}{76.6}            & 0             & \multicolumn{1}{c|}{7.09}             & 4.93          & \multicolumn{1}{c|}{69}          & 36       & \multicolumn{1}{c|}{64}          & 31       & \multicolumn{1}{c|}{15.25}       & 36.73    \\ \hline
PC/YAGO      & \multicolumn{1}{c|}{55299}    & 42016  & \multicolumn{1}{c|}{11.4}          & 55.3       & \multicolumn{1}{c|}{14.8}            & 0             & \multicolumn{1}{c|}{7.46}             & 3.54          & \multicolumn{1}{c|}{85}          & 27       & \multicolumn{1}{c|}{80}          & 22       & \multicolumn{1}{c|}{79.28}       & 96.1    \\ \hline
PV/DBLP  & \multicolumn{1}{c|}{40618}    & 44886  & \multicolumn{1}{c|}{29.94}         & 65.37      & \multicolumn{1}{c|}{0}               & 0             & \multicolumn{1}{c|}{4.05}             & 3.65          & \multicolumn{1}{c|}{34}          & 33       & \multicolumn{1}{c|}{33}          & 34       & \multicolumn{1}{c|}{81.79}       & 80.53      \\ \hline
PV/MAG   & \multicolumn{1}{c|}{36149}     & 44956   & \multicolumn{1}{c|}{4.90}          & 78.0       & \multicolumn{1}{c|}{89.27}            & 0             & \multicolumn{1}{c|}{3.00}              & 2.99           & \multicolumn{1}{c|}{48}          & 20        & \multicolumn{1}{c|}{43}          & 22        & \multicolumn{1}{c|}{73.79 }   &   75.33 \\ \hline
\end{tabular}
\vspace*{-2ex}
\end{table*}

==> tables/table_subgraphs_statistics.tex <==
\begin{table}[t]\centering
\caption{DBLP sub-graph datasets statistics}
\label{tbl_DBLP_subgraph_datasets_statistics}
% \renewcommand{\arraystretch}{1.5}
\scriptsize
\begin{tabular}{|p{10em}|p{3.5em}|p{4.5em}|p{2em}|p{2em}|p{4em}|p{2em}|}
\toprule
Sub-graph&\#Nodes V&\#Targets Nodes $V^t$ &\#Node Types&\#Edge Types&\#Triples&$\frac{|V|}{|V^t|}$
\\\midrule
FG (Full Graph)&15,607,309 &1,123,344 &43 &41 &29,643,988 &1.90 
\\
% \midrule
RS (Relevant sub-graph) &3,421,568 &1,123,344 &3 &2 &5,374,099 &1.57 
\\
% \midrule
GA (Genetic Algorithm sub-graph)  &3,570,895 &1,123,344 &11 &10 &7,638,586 &2.14
\\
% % \midrule
% GA2 &2,257,948 &1,123,344 &7 &6 &5,816,085 &2.58 \\
\bottomrule
\end{tabular}
\end{table}
